The Boundary Layer in compact binaries

We perform numerical hydrodynamical simulations in order to calculate the luminosity and the spectrum of the BL and its dependence on parameters like the mass, rotation rate or mass accretion rate of the central white dwarf (WD). Therefore, we treat the problem in the one-dimensional, radial slim disk approximation. We employ a classical $\alpha$-viscosity to account for the turbulence and include cooling from the disk surfaces as well as radial radiation transport. To account for the high temperatures in BLs around WDs, we also consider the radiation energy in a one-temperature approximation. We find that 1D models of the BL are well suited if one is interested in the radiation characteristics of the BL. The BL luminosity directly depends on the varied parameters which makes it possible to draw conclusions about real systems by comparing observations with our synthetic models. Ambiguities concerning different models with identical luminosities can be mitigated by regarding the emitted spectrum. We therefore present a method to gain information about a system by probing the radiation of the BL.

==> references <==
@ARTICLE{1997MNRAS.285..239K,
   author = {{Kley}, W. and {Papaloizou}, J.~C.~B.},
    title = "{Causal Viscosity in Accretion Disc Boundary layers}",
  journal = {\mnras},
 keywords = {ACCRETION, ACCRETION DISCS: HYDRODYNAMICS},
     year = 1997,
    month = feb,
   volume = 285,
    pages = {239-252},
   adsurl = {http://adsabs.harvard.edu/abs/1997MNRAS.285..239K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1987ARA&A..25...23S,
   author = {{Shu}, F.~H. and {Adams}, F.~C. and {Lizano}, S.},
    title = "{Star formation in molecular clouds - Observation and theory}",
  journal = {\araa},
 keywords = {ASTROPHYSICS, MOLECULAR CLOUDS, STAR FORMATION, STELLAR MODELS, ASTRONOMICAL MAPS, BINARY STARS, GRAVITATIONAL COLLAPSE, PROTOSTARS, STAR CLUSTERS, STELLAR
MASS},
     year = 1987,
   volume = 25,
    pages = {23-81},
      doi = {10.1146/annurev.aa.25.090187.000323},
   adsurl = {http://adsabs.harvard.edu/abs/1987ARA%26A..25...23S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1986MNRAS.221..279R,
   author = {{Robertson}, J.~A. and {Frank}, J.},
    title = "{A numerical study of two-dimensional accretion flows}",
  journal = {\mnras},
 keywords = {ACCRETION DISKS, COMPUTATIONAL ASTROPHYSICS, HYDRODYNAMIC EQUATIONS, STELLAR MASS ACCRETION, TWO DIMENSIONAL FLOW, ADVECTION, ALTERNATING DIRECTION IMPLICIT
METHODS, CIRCULAR CYLINDERS, ENERGY DISSIPATION, INCOMPRESSIBLE FLOW, STEADY FLOW, STELLAR EVOLUTION},
     year = 1986,
    month = jul,
   volume = 221,
    pages = {279-309},
   adsurl = {http://adsabs.harvard.edu/abs/1986MNRAS.221..279R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1987A&A...172..124K,
   author = {{Kley}, W. and {Hensler}, G.},
    title = "{Two-dimensional numerical models of the boundary layer of accretion disks in cataclysmic variables}",
  journal = {\aap},
 keywords = {ACCRETION DISKS, BOUNDARY LAYER FLOW, CATACLYSMIC VARIABLES, STELLAR MODELS, STELLAR ROTATION, TWO DIMENSIONAL FLOW, TWO DIMENSIONAL MODELS, ADVECTION,
ENERGY DISSIPATION, SPECTRAL ENERGY DISTRIBUTION, STELLAR STRUCTURE},
     year = 1987,
    month = jan,
   volume = 172,
    pages = {124-142},
   adsurl = {http://adsabs.harvard.edu/abs/1987A%26A...172..124K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1989A&A...208...98K,
   author = {{Kley}, W.},
    title = "{Radiation hydrodynamics of the boundary layer in accretion disks. I - Numerical methods}",
  journal = {\aap},
 keywords = {ACCRETION DISKS, CATACLYSMIC VARIABLES, COMPUTATIONAL ASTROPHYSICS, MAGNETOHYDRODYNAMICS, ANGULAR MOMENTUM, RADIATION TRANSPORT, VISCOUS FLOW, WHITE DWARF
STARS},
     year = 1989,
    month = jan,
   volume = 208,
    pages = {98-110},
   adsurl = {http://adsabs.harvard.edu/abs/1989A%26A...208...98K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1989A&A...222..141K,
   author = {{Kley}, W.},
    title = "{Radiation hydrodynamics of the boundary layer in accretion disks. II - Optically thick models}",
  journal = {\aap},
 keywords = {ACCRETION DISKS, CATACLYSMIC VARIABLES, COMPUTATIONAL ASTROPHYSICS, HYDRODYNAMICS, STELLAR MODELS, WHITE DWARF STARS, ANGULAR VELOCITY, BOUNDARY LAYERS,
RADIATION DISTRIBUTION, STELLAR CORONAS, STELLAR ROTATION},
     year = 1989,
    month = sep,
   volume = 222,
    pages = {141-149},
   adsurl = {http://adsabs.harvard.edu/abs/1989A%26A...222..141K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{liddle2003introduction,
  title={An introduction to modern cosmology},
  author={Liddle, A.R.},
  isbn={9780470848340},
  lccn={2003269979},
  url={http://books.google.de/books?id=cxcpAQAAMAAJ},
  year={2003},
  publisher={Wiley}
}

@BOOK{perkins2009particle,
  title={Particle Astrophysics},
  author={Perkins, D.H.},
  isbn={9780199545452},
  lccn={2008049651},
  series={Oxford master series in physics: Particle physics, astrophysics, and cosmology},
  url={http://books.google.de/books?id=fBNzZF7kLz4C},
  year={2009},
  publisher={Oxford University Press}
}

@ARTICLE{1902RSPTA.199....1J,
   author = {{Jeans}, J.~H.},
    title = "{The Stability of a Spherical Nebula}",
  journal = {Royal Society of London Philosophical Transactions Series A},
     year = 1902,
   volume = 199,
    pages = {1-53},
      doi = {10.1098/rsta.1902.0012},
   adsurl = {http://adsabs.harvard.edu/abs/1902RSPTA.199....1J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1993prpl.conf..497H,
   author = {{Hartmann}, L. and {Kenyon}, S. and {Hartigan}, P.},
    title = "{Young stars - Episodic phenomena, activity and variability}",
 keywords = {PRE-MAIN SEQUENCE STARS, STAR FORMATION RATE, STELLAR MASS ACCRETION, STELLAR PHYSICS, EARLY STARS, T TAURI STARS, VARIABILITY},
booktitle = {Protostars and Planets III},
     year = 1993,
   editor = {{Levy}, E.~H. and {Lunine}, J.~I.},
    pages = {497-518},
   adsurl = {http://adsabs.harvard.edu/abs/1993prpl.conf..497H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1990AJ.....99..924B,
   author = {{Beckwith}, S.~V.~W. and {Sargent}, A.~I. and {Chini}, R.~S. and 
	{Guesten}, R.},
    title = "{A survey for circumstellar disks around young stellar objects}",
  journal = {\aj},
 keywords = {MOLECULAR CLOUDS, PRE-MAIN SEQUENCE STARS, SKY SURVEYS (ASTRONOMY), STELLAR ENVELOPES, T TAURI STARS, AURIGA CONSTELLATION, COMPUTATIONAL ASTROPHYSICS,
EMISSION SPECTRA, H ALPHA LINE, MILKY WAY GALAXY, STELLAR EVOLUTION, TAURUS CONSTELLATION},
     year = 1990,
    month = mar,
   volume = 99,
    pages = {924-945},
      doi = {10.1086/115385},
   adsurl = {http://adsabs.harvard.edu/abs/1990AJ.....99..924B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{frank2002accretion,
  title={Accretion Power in Astrophysics},
  author={Frank, J. and King, A.R. and Raine, D.J.},
  isbn={9780521629577},
  lccn={2001037846},
  url={http://books.google.de/books?id=GGM\_t-xn8ocC},
  year={2002},
  publisher={Cambridge University Press}
}

@ARTICLE{1981MNRAS.194..809L,
   author = {{Larson}, R.~B.},
    title = "{Turbulence and star formation in molecular clouds}",
  journal = {\mnras},
 keywords = {INTERSTELLAR MATTER, MOLECULAR CLOUDS, PROTOSTARS, STAR FORMATION, TURBULENCE EFFECTS, CLUMPS, DENSITY DISTRIBUTION, STELLAR GRAVITATION, STELLAR MASS,
VELOCITY DISTRIBUTION, VIRIAL THEOREM},
     year = 1981,
    month = mar,
   volume = 194,
    pages = {809-826},
   adsurl = {http://adsabs.harvard.edu/abs/1981MNRAS.194..809L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007ARA&A..45..565M,
   author = {{McKee}, C.~F. and {Ostriker}, E.~C.},
    title = "{Theory of Star Formation}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {0707.3514},
     year = 2007,
    month = sep,
   volume = 45,
    pages = {565-687},
      doi = {10.1146/annurev.astro.45.051806.110602},
   adsurl = {http://adsabs.harvard.edu/abs/2007ARA%26A..45..565M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1993ApJ...406..528G,
   author = {{Goodman}, A.~A. and {Benson}, P.~J. and {Fuller}, G.~A. and 
	{Myers}, P.~C.},
    title = "{Dense cores in dark clouds. VIII - Velocity gradients}",
  journal = {\apj},
 keywords = {ANGULAR VELOCITY, MOLECULAR CLOUDS, STAR FORMATION, STELLAR MOTIONS, VELOCITY DISTRIBUTION, ANGULAR MOMENTUM, GRADIENTS},
     year = 1993,
    month = apr,
   volume = 406,
    pages = {528-547},
      doi = {10.1086/172465},
   adsurl = {http://adsabs.harvard.edu/abs/1993ApJ...406..528G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1995Natur.378..355M,
   author = {{Mayor}, M. and {Queloz}, D.},
    title = "{A Jupiter-mass companion to a solar-type star}",
  journal = {\nat},
     year = 1995,
    month = nov,
   volume = 378,
    pages = {355-359},
      doi = {10.1038/378355a0},
   adsurl = {http://adsabs.harvard.edu/abs/1995Natur.378..355M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1996Icar..124...62P,
   author = {{Pollack}, J.~B. and {Hubickyj}, O. and {Bodenheimer}, P. and 
	{Lissauer}, J.~J. and {Podolak}, M. and {Greenzweig}, Y.},
    title = "{Formation of the Giant Planets by Concurrent Accretion of Solids and Gas}",
  journal = {\icarus},
     year = 1996,
    month = nov,
   volume = 124,
    pages = {62-85},
      doi = {10.1006/icar.1996.0190},
   adsurl = {http://adsabs.harvard.edu/abs/1996Icar..124...62P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007prpl.conf..607D,
   author = {{Durisen}, R.~H. and {Boss}, A.~P. and {Mayer}, L. and {Nelson}, A.~F. and 
	{Quinn}, T. and {Rice}, W.~K.~M.},
    title = "{Gravitational Instabilities in Gaseous Protoplanetary Disks and Implications for Giant Planet Formation}",
  journal = {Protostars and Planets V},
   eprint = {arXiv:astro-ph/0603179},
     year = 2007,
    pages = {607-622},
   adsurl = {http://adsabs.harvard.edu/abs/2007prpl.conf..607D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1999ApJ...525..330Y,
   author = {{Yorke}, H.~W. and {Bodenheimer}, P.},
    title = "{The Formation of Protostellar Disks. III. The Influence of Gravitationally Induced Angular Momentum Transport on Disk Structure and Appearance}",
  journal = {\apj},
 keywords = {HYDRODYNAMICS, ISM: CLOUDS, RADIATIVE TRANSFER, STARS: FORMATION},
     year = 1999,
    month = nov,
   volume = 525,
    pages = {330-342},
      doi = {10.1086/307867},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...525..330Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005ApJ...635..396E,
   author = {{Eisner}, J.~A. and {Hillenbrand}, L.~A. and {Carpenter}, J.~M. and 
	{Wolf}, S.},
    title = "{Constraining the Evolutionary Stage of Class I Protostars: Multiwavelength Observations and Modeling}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0508380},
 keywords = {Stars: Circumstellar Matter, Stars: Formation, Stars: Individual: Alphanumeric: IRAS 04016+2610, stars: individual (IRAS 04108+2803B), stars: individual
(IRAS 04239+2436), stars: individual (IRAS 04295+2251), stars: individual (IRAS 04381+2540), Techniques: High Anular Resolution},
     year = 2005,
    month = dec,
   volume = 635,
    pages = {396-421},
      doi = {10.1086/497161},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...635..396E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1998AJ....116..854B,
   author = {{Bally}, J. and {Testi}, L. and {Sargent}, A. and {Carlstrom}, J.
	},
    title = "{Disk Mass Limits and Lifetimes of Externally Irradiated Young Stellar Objects Embedded in the Orion Nebula}",
  journal = {\aj},
 keywords = {ISM: INDIVIDUAL: NAME: ORION NEBULA, STARS: GENERAL, STARS: PRE-MAIN-SEQUENCE},
     year = 1998,
    month = aug,
   volume = 116,
    pages = {854-859},
      doi = {10.1086/300469},
   adsurl = {http://adsabs.harvard.edu/abs/1998AJ....116..854B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001ApJ...553L.153H,
   author = {{Haisch}, Jr., K.~E. and {Lada}, E.~A. and {Lada}, C.~J.},
    title = "{Disk Frequencies and Lifetimes in Young Clusters}",
  journal = {\apjl},
   eprint = {arXiv:astro-ph/0104347},
 keywords = {Infrared: Stars, Galaxy: Open Clusters and Associations: General, Stars: Planetary Systems: Protoplanetary Disks, Stars: Formation},
     year = 2001,
    month = jun,
   volume = 553,
    pages = {L153-L156},
      doi = {10.1086/320685},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...553L.153H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001Sci...291...93B,
   author = {{Brice{\~n}o}, C. and {Vivas}, A.~K. and {Calvet}, N. and {Hartmann}, L. and 
	{Pacheco}, R. and {Herrera}, D. and {Romero}, L. and {Berlind}, P. and 
	{S{\'a}nchez}, G. and {Snyder}, J.~A. and {Andrews}, P.},
    title = "{The CIDA-QUEST Large-Scale Survey of Orion OB1: Evidence for Rapid Disk Dissipation in a Dispersed Stellar Population}",
  journal = {Science},
     year = 2001,
    month = jan,
   volume = 291,
    pages = {93-97},
      doi = {10.1126/science.291.5501.93},
   adsurl = {http://adsabs.harvard.edu/abs/2001Sci...291...93B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003ApJ...598.1341E,
   author = {{Eisner}, J.~A. and {Carpenter}, J.~M.},
    title = "{Distribution of Circumstellar Disk Masses in the Young Cluster NGC 2024}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0308279},
 keywords = {Galaxy: Open Clusters and Associations: Individual: NGC Number: NGC 2024, Stars: Planetary Systems: Protoplanetary Disks, Stars: Pre-Main-Sequence},
     year = 2003,
    month = dec,
   volume = 598,
    pages = {1341-1349},
      doi = {10.1086/379102},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...598.1341E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000MNRAS.318...18N,
   author = {{Nelson}, R.~P. and {Papaloizou}, J.~C.~B. and {Masset}, F. and 
	{Kley}, W.},
    title = "{The migration and growth of protoplanets in protostellar discs}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/9909486},
 keywords = {ACCRETION, ACCRETION DISCS, METHODS: NUMERICAL, PLANETS AND SATELLITES: GENERAL, SOLAR SYSTEM: FORMATION, PLANETARY SYSTEMS},
     year = 2000,
    month = oct,
   volume = 318,
    pages = {18-36},
      doi = {10.1046/j.1365-8711.2000.03605.x},
   adsurl = {http://adsabs.harvard.edu/abs/2000MNRAS.318...18N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003MNRAS.341..213B,
   author = {{Bate}, M.~R. and {Lubow}, S.~H. and {Ogilvie}, G.~I. and {Miller}, K.~A.
	},
    title = "{Three-dimensional calculations of high- and low-mass planets embedded in protoplanetary discs}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/0301154},
 keywords = {accretion, accretion discs, hydrodynamics, planets and satellites: formation, planetary systems: formation, planetary systems: protoplanetary discs},
     year = 2003,
    month = may,
   volume = 341,
    pages = {213-229},
      doi = {10.1046/j.1365-8711.2003.06406.x},
   adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.341..213B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1977MNRAS.180...57W,
   author = {{Weidenschilling}, S.~J.},
    title = "{Aerodynamics of solid bodies in the solar nebula}",
  journal = {\mnras},
 keywords = {AERODYNAMIC DRAG, INTERPLANETARY DUST, NEBULAE, RADIAL VELOCITY, SOLIDS, SUN, EQUATIONS OF MOTION, FRACTIONATION, ORBITAL VELOCITY, PARTICLE COLLISIONS,
PARTICLE MOTION, PRESSURE GRADIENTS, STELLAR MODELS, WIND VELOCITY},
     year = 1977,
    month = jul,
   volume = 180,
    pages = {57-70},
   adsurl = {http://adsabs.harvard.edu/abs/1977MNRAS.180...57W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{1971cgat.book.....M,
   author = {{Martynov}, D.~Y.},
    title = "{Course of general astrophysics. Text-book for students of astronomy.}",
     year = 1971,
   adsurl = {http://adsabs.harvard.edu/abs/1971cgat.book.....M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System},
publisher = {Nauka, Moskva}
}

%booktitle = {Course of general astrophysics.~Text-book for students of astronomy., by Martynov, D.~Ya..~ Second edition.~Moskva: Nauka, 616 p.},

@ARTICLE{1970PASP...82..809J,
   author = {{Jaschek}, C. and {G{\'o}mez}, A.~E.},
    title = "{The Frequency of Spectroscopic Binaries}",
  journal = {\pasp},
     year = 1970,
    month = aug,
   volume = 82,
    pages = {809},
      doi = {10.1086/128966},
   adsurl = {http://adsabs.harvard.edu/abs/1970PASP...82..809J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1967oeds.conf...44V,
   author = {{van Albada}, T.~S. and {Blaauw}, A.},
    title = "{D{\'e}finition de l'objet ''{\'e}toile double'': On the frequency distribution of separations and mass ratios of early-type double stars}",
booktitle = {On the Evolution of Double Stars},
     year = 1967,
   editor = {{Dommanget}, J.},
    pages = {44},
   adsurl = {http://adsabs.harvard.edu/abs/1967oeds.conf...44V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1971ARA&A...9..183P,
   author = {{Paczy{\'n}ski}, B.},
    title = "{Evolutionary Processes in Close Binary Systems}",
  journal = {\araa},
     year = 1971,
   volume = 9,
    pages = {183},
      doi = {10.1146/annurev.aa.09.090171.001151},
   adsurl = {http://adsabs.harvard.edu/abs/1971ARA%26A...9..183P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010MNRAS.403...45S,
   author = {{Stacy}, A. and {Greif}, T.~H. and {Bromm}, V.},
    title = "{The first stars: formation of binaries and small multiple systems}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0908.0712},
 primaryClass = "astro-ph.CO",
 keywords = {stars: formation, galaxies: formation, cosmology: theory, early Universe},
     year = 2010,
    month = mar,
   volume = 403,
    pages = {45-60},
      doi = {10.1111/j.1365-2966.2009.16113.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.403...45S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1963AcA....13..106K,
   author = {{Kruszewski}, A.},
    title = "{Exchange of Matter in Close Binary Systems. I. Equilibrium Configurations in the Case of Deviations from Synchronism}",
  journal = {\actaa},
     year = 1963,
   volume = 13,
    pages = {106},
   adsurl = {http://adsabs.harvard.edu/abs/1963AcA....13..106K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1976ApJ...209..536S,
   author = {{Shu}, F.~H. and {Lubow}, S.~H. and {Anderson}, L.},
    title = "{On the structure of contact binaries. I - The contact discontinuity}",
  journal = {\apj},
 keywords = {BINARY STARS, STELLAR STRUCTURE, DISCONTINUITY, DYNAMIC STABILITY, STELLAR ENVELOPES, STELLAR MODELS, STELLAR TEMPERATURE, THERMAL DIFFUSION},
     year = 1976,
    month = oct,
   volume = 209,
    pages = {536-546},
      doi = {10.1086/154748},
   adsurl = {http://adsabs.harvard.edu/abs/1976ApJ...209..536S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1977ApJ...216..517L,
   author = {{Lubow}, S.~H. and {Shu}, F.~H.},
    title = "{On the structure of contact binaries. II - Zero-age models}",
  journal = {\apj},
 keywords = {CONVECTIVE FLOW, ECLIPSING BINARY STARS, STELLAR MODELS, STELLAR STRUCTURE, CHEMICAL COMPOSITION, MAIN SEQUENCE STARS, STELLAR ATMOSPHERES, STELLAR
ENVELOPES, STELLAR LUMINOSITY, STELLAR MASS, STELLAR TEMPERATURE},
     year = 1977,
    month = sep,
   volume = 216,
    pages = {517-525},
      doi = {10.1086/155493},
   adsurl = {http://adsabs.harvard.edu/abs/1977ApJ...216..517L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1979ApJ...229..223S,
   author = {{Shu}, F.~H. and {Anderson}, L. and {Lubow}, S.~H.},
    title = "{On the structure of contact binaries. III - Mass and energy flow}",
  journal = {\apj},
 keywords = {BINARY STARS, DISCONTINUITY, ENERGY TRANSFER, HYDRODYNAMICS, MASS FLOW, STELLAR STRUCTURE, GAS DYNAMICS, QUALITATIVE ANALYSIS, STELLAR EVOLUTION, STELLAR
LUMINOSITY, TRANSITION LAYERS, TURBULENT MIXING},
     year = 1979,
    month = apr,
   volume = 229,
    pages = {223-241},
      doi = {10.1086/156948},
   adsurl = {http://adsabs.harvard.edu/abs/1979ApJ...229..223S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1970IAUS...39..272P,
   author = {{Pottasch}, S.~R.},
    title = "{Mass Loss from Stars}",
booktitle = {Interstellar Gas Dynamics},
     year = 1970,
   series = {IAU Symposium},
   volume = 39,
   editor = {{Habing}, H.~J.},
    pages = {272},
   adsurl = {http://adsabs.harvard.edu/abs/1970IAUS...39..272P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1977ApJ...216..822P,
   author = {{Paczynski}, B.},
    title = "{A model of accretion disks in close binaries}",
  journal = {\apj},
 keywords = {BINARY STARS, STELLAR MASS ACCRETION, STELLAR MODELS, ASTRONOMICAL MODELS, DISKS (SHAPES), HYDRODYNAMICS, RADIAL VELOCITY, THREE BODY PROBLEM},
     year = 1977,
    month = sep,
   volume = 216,
    pages = {822-826},
      doi = {10.1086/155526},
   adsurl = {http://adsabs.harvard.edu/abs/1977ApJ...216..822P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1983AcA....33..319G,
   author = {{Giovannelli}, F. and {Gaudenzi}, S. and {Rossi}, C. and {Piccioni}, A.
	},
    title = "{Orbital parameters of SS Cygni}",
  journal = {\actaa},
 keywords = {DWARF NOVAE, LINE SPECTRA, ORBITAL ELEMENTS, STELLAR SPECTROPHOTOMETRY, BALMER SERIES, BREMSSTRAHLUNG, H LINES, K LINES},
     year = 1983,
   volume = 33,
    pages = {319-330},
   adsurl = {http://adsabs.harvard.edu/abs/1983AcA....33..319G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1994A&A...291..455M,
   author = {{Martinez-Pais}, I.~G. and {Giovannelli}, F. and {Rossi}, C. and 
	{Gaudenzi}, S.},
    title = "{An optical time-resolved spectroscopic study of SS Cygni. 1: Quiescence}",
  journal = {\aap},
 keywords = {ABSORPTION SPECTRA, ACCRETION DISKS, CATACLYSMIC VARIABLES, MAIN SEQUENCE STARS, STELLAR SPECTRA, TEMPORAL RESOLUTION, WHITE DWARF STARS, BALMER SERIES, H
ALPHA LINE, IRON, RADIAL VELOCITY},
     year = 1994,
    month = nov,
   volume = 291,
    pages = {455-467},
   adsurl = {http://adsabs.harvard.edu/abs/1994A%26A...291..455M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1974MNRAS.168..603L,
   author = {{Lynden-Bell}, D. and {Pringle}, J.~E.},
    title = "{The evolution of viscous discs and the origin of the nebular variables.}",
  journal = {\mnras},
     year = 1974,
    month = sep,
   volume = 168,
    pages = {603-637},
   adsurl = {http://adsabs.harvard.edu/abs/1974MNRAS.168..603L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@MASTERSTHESIS{Mueller2010,
	author = {{Müller}, Tobias W.~A.},
	title  = "{Self-gravitating Accretion Disks}",
	school = {Eberhard Karls Universität Tübingen},
	year   = 2010,
	moth   = feb
}

@ARTICLE{1999MNRAS.303..696K,
   author = {{Kley}, W.},
    title = "{Mass flow and accretion through gaps in accretion discs}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/9809253},
 keywords = {ACCRETION, ACCRETION DISCS, HYDRODYNAMICS, PLANETS AND SATELLITES: GENERAL, STARS: FORMATION, PLANETARY SYSTEMS},
     year = 1999,
    month = mar,
   volume = 303,
    pages = {696-710},
      doi = {10.1046/j.1365-8711.1999.02198.x},
   adsurl = {http://adsabs.harvard.edu/abs/1999MNRAS.303..696K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000A&AS..141..165M,
   author = {{Masset}, F.},
    title = "{FARGO: A fast eulerian transport algorithm for differentially rotating disks}",
  journal = {\aaps},
   eprint = {arXiv:astro-ph/9910390},
 keywords = {ACCRETION, ACCRETION DISKS, HYDRODYNAMICS, METHODS: NUMERICAL},
     year = 2000,
    month = jan,
   volume = 141,
    pages = {165-173},
      doi = {10.1051/aas:2000116},
   adsurl = {http://adsabs.harvard.edu/abs/2000A%26AS..141..165M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1978JCoPh..27....1S,
   author = {{Sod}, G.~A.},
    title = "{A survey of several finite difference methods for systems of nonlinear hyperbolic conservation laws}",
  journal = {J.~Comput.~Phys.},
 keywords = {CONSERVATION LAWS, FINITE DIFFERENCE THEORY, FLOW EQUATIONS, GAS FLOW, HYPERBOLIC DIFFERENTIAL EQUATIONS, NONLINEAR EQUATIONS, CARTESIAN COORDINATES, FLOW
THEORY, GAS DYNAMICS, ONE DIMENSIONAL FLOW, SHOCK TUBES},
     year = 1978,
    month = apr,
   volume = 27,
    pages = {1-31},
      doi = {10.1016/0021-9991(78)90023-2},
   adsurl = {http://adsabs.harvard.edu/abs/1978JCoPh..27....1S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1984ApJ...277..296H,
   author = {{Hawley}, J.~F. and {Smarr}, L.~L. and {Wilson}, J.~R.},
    title = "{A numerical study of nonspherical black hole accretion. I Equations and test problems}",
  journal = {\apj},
 keywords = {ASTRONOMICAL MODELS, BLACK HOLES (ASTRONOMY), HYDRODYNAMICS, STELLAR MASS ACCRETION, COMPUTATIONAL FLUID DYNAMICS, HYDRODYNAMIC EQUATIONS, RELATIVITY, SHOCK
WAVES, TRANSONIC FLOW},
     year = 1984,
    month = feb,
   volume = 277,
    pages = {296-311},
      doi = {10.1086/161696},
   adsurl = {http://adsabs.harvard.edu/abs/1984ApJ...277..296H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1984ApJS...55..211H,
   author = {{Hawley}, J.~F. and {Smarr}, L.~L. and {Wilson}, J.~R.},
    title = "{A numerical study of nonspherical black hole accretion. II - Finite differencing and code calibration}",
  journal = {\apjs},
 keywords = {BLACK HOLES (ASTRONOMY), COMPUTATIONAL FLUID DYNAMICS, FINITE DIFFERENCE THEORY, GAS DYNAMICS, STELLAR MASS ACCRETION, CALIBRATING, CODES, COSMIC DUST,
HYDRODYNAMIC EQUATIONS, INVISCID FLOW, RELATIVISTIC EFFECTS, SHOCK TUBES},
     year = 1984,
    month = jun,
   volume = 55,
    pages = {211-246},
      doi = {10.1086/190953},
   adsurl = {http://adsabs.harvard.edu/abs/1984ApJS...55..211H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008MNRAS.390.1267T,
   author = {{Tasker}, E.~J. and {Brunino}, R. and {Mitchell}, N.~L. and 
	{Michielsen}, D. and {Hopton}, S. and {Pearce}, F.~R. and {Bryan}, G.~L. and 
	{Theuns}, T.},
    title = "{A test suite for quantitative comparison of hydrodynamic codes in astrophysics}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0808.1844},
 keywords = {hydrodynamics , methods: numerical , cosmology: theory},
     year = 2008,
    month = nov,
   volume = 390,
    pages = {1267-1281},
      doi = {10.1111/j.1365-2966.2008.13836.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.390.1267T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{1959sdmm.book.....S,
   author = {{Sedov}, L.~I.},
    title = "{Similarity and Dimensional Methods in Mechanics}",
     year = 1959,
   adsurl = {http://adsabs.harvard.edu/abs/1959sdmm.book.....S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System},
publisher = {CRC Press}
}

booktitle = {Similarity and Dimensional Methods in Mechanics, New York: Academic Press, 1959},

@BOOK{1959flme.book.....L,
   author = {{Landau}, L.~D. and {Lifshitz}, E.~M.},
    title = "{Fluid mechanics}",
booktitle = {Course of theoretical physics},
     year = 1959,
   adsurl = {http://adsabs.harvard.edu/abs/1959flme.book.....L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System},
publisher = {Pergamon Press, Oxford}
}

@ARTICLE{2008A&A...487L...9K,
   author = {{Kley}, W. and {Crida}, A.},
    title = "{Migration of protoplanets in radiative discs}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0806.2990},
 keywords = {stars: planetary systems: formation, accretion, accretion disks},
     year = 2008,
    month = aug,
   volume = 487,
    pages = {L9-L12},
      doi = {10.1051/0004-6361:200810033},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...487L...9K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1979ApJS...41..743C,
   author = {{Cohen}, M. and {Kuhi}, L.~V.},
    title = "{Observational studies of pre-main-sequence evolution}",
  journal = {\apjs},
 keywords = {MAIN SEQUENCE STARS, STELLAR EVOLUTION, STELLAR SPECTRA, STELLAR SPECTROPHOTOMETRY, ASTRONOMICAL CATALOGS, BINARY STARS, EMISSION SPECTRA,
HERTZSPRUNG-RUSSELL DIAGRAM, INFRARED ASTRONOMY, LINE SPECTRA, OPTICAL SCANNERS, STELLAR LUMINOSITY, STELLAR TEMPERATURE},
     year = 1979,
    month = dec,
   volume = 41,
    pages = {743-843},
      doi = {10.1086/190641},
   adsurl = {http://adsabs.harvard.edu/abs/1979ApJS...41..743C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1994ApJ...435..821L,
   author = {{Lin}, D.~N.~C. and {Hayashi}, M. and {Bell}, K.~R. and {Ohashi}, N.
	},
    title = "{Is HL Tauri and FU Orionis system in quiescence?}",
  journal = {\apj},
 keywords = {ACCRETION DISKS, KEPLER LAWS, PRE-MAIN SEQUENCE STARS, STELLAR EVOLUTION, STELLAR LUMINOSITY, STELLAR MODELS, DEPOSITION, MATHEMATICAL MODELS, STELLAR
ENVELOPES},
     year = 1994,
    month = nov,
   volume = 435,
    pages = {821-828},
      doi = {10.1086/174861},
   adsurl = {http://adsabs.harvard.edu/abs/1994ApJ...435..821L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1996ApJ...461..933K,
   author = {{Kley}, W. and {Lin}, D.~N.~C.},
    title = "{The Structure of the Boundary Layer in Protostellar Disks}",
  journal = {\apj},
 keywords = {STARS: CIRCUMSTELLAR MATTER, HYDRODYNAMICS, STARS: FORMATION, STARS: PRE-MAIN-SEQUENCE},
     year = 1996,
    month = apr,
   volume = 461,
    pages = {933},
      doi = {10.1086/177115},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...461..933K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1991ApJ...370..604P,
   author = {{Popham}, R. and {Narayan}, R.},
    title = "{Does accretion cease when a star approaches breakup?}",
  journal = {\apj},
 keywords = {ACCRETION DISKS, BINARY STARS, STELLAR MASS ACCRETION, STELLAR ROTATION, WHITE DWARF STARS, ANGULAR MOMENTUM, BOUNDARY CONDITIONS, HYDRODYNAMICS, NUMERICAL
ANALYSIS, RADIAL VELOCITY, STAR FORMATION, SUBSONIC FLOW, SUPERSONIC FLOW},
     year = 1991,
    month = apr,
   volume = 370,
    pages = {604-614},
      doi = {10.1086/169847},
   adsurl = {http://adsabs.harvard.edu/abs/1991ApJ...370..604P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001ApJ...553..174G,
   author = {{Gammie}, C.~F.},
    title = "{Nonlinear Outcome of Gravitational Instability in Cooling, Gaseous Disks}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0101501},
 keywords = {Accretion, Accretion Disks, Galaxies: Nuclei, Solar System: Formation},
     year = 2001,
    month = may,
   volume = 553,
    pages = {174-183},
      doi = {10.1086/320631},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...553..174G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1998RvMP...70....1B,
   author = {{Balbus}, S.~A. and {Hawley}, J.~F.},
    title = "{Instability, turbulence, and enhanced transport in accretion disks}",
  journal = {Rev.~Mod.~Phys.},
 keywords = {Accretion and accretion disks, Hydrodynamics, Infall, accretion, and accretion disks, Plasma dynamics and flow, Plasma turbulence, Magnetohydrodynamics and
plasmas},
     year = 1998,
    month = jan,
   volume = 70,
    pages = {1-53},
      doi = {10.1103/RevModPhys.70.1},
   adsurl = {http://adsabs.harvard.edu/abs/1998RvMP...70....1B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009ApJ...702.1536B,
   author = {{Balsara}, D.~S. and {Fisker}, J.~L. and {Godon}, P. and {Sion}, E.~M.
	},
    title = "{Simulations of the Boundary Layer Between a White Dwarf and Its Accretion Disk}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0705.2582},
 keywords = {accretion, accretion disks, binaries: close, methods: numerical, novae, cataclysmic variables, white dwarfs},
     year = 2009,
    month = sep,
   volume = 702,
    pages = {1536-1552},
      doi = {10.1088/0004-637X/702/2/1536},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...702.1536B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004ApJ...603..401T,
   author = {{Tan}, J.~C. and {Blackman}, E.~G.},
    title = "{Protostellar Disk Dynamos and Hydromagnetic Outflows in Primordial Star Formation}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0307455},
 keywords = {Cosmology: Early Universe, Magnetohydrodynamics: MHD, Stars: Formation, Stars: Magnetic Fields, Stars: Winds, Outflows},
     year = 2004,
    month = mar,
   volume = 603,
    pages = {401-413},
      doi = {10.1086/381668},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...603..401T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1995ApJ...438..813S,
   author = {{Strom}, K.~M. and {Kepner}, J. and {Strom}, S.~E.},
    title = "{The evolutionary status of the stellar population in the rho Ophiuchi cloud core}",
  journal = {\apj},
 keywords = {MOLECULAR CLOUDS, POPULATIONS, PRE-MAIN SEQUENCE STARS, SKY SURVEYS (ASTRONOMY), STAR FORMATION, INFRARED IMAGERY, STELLAR ENVELOPES, STELLAR MASS, STELLAR
PHYSICS, STELLAR WINDS},
     year = 1995,
    month = jan,
   volume = 438,
    pages = {813-829},
      doi = {10.1086/175125},
   adsurl = {http://adsabs.harvard.edu/abs/1995ApJ...438..813S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1993prpl.conf..543B,
   author = {{Basri}, G. and {Bertout}, C.},
    title = "{T Tauri stars and their accretion disks}",
 keywords = {ACCRETION DISKS, PRE-MAIN SEQUENCE STARS, STELLAR MODELS, STELLAR RADIATION, T TAURI STARS, H ALPHA LINE, STELLAR ENVELOPES, STELLAR SPECTRA},
booktitle = {Protostars and Planets III},
     year = 1993,
   editor = {{Levy}, E.~H. and {Lunine}, J.~I.},
    pages = {543-566},
   adsurl = {http://adsabs.harvard.edu/abs/1993prpl.conf..543B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1980MNRAS.191...37L,
   author = {{Lin}, D.~N.~C. and {Papaloizou}, J.},
    title = "{On the structure and evolution of the primordial solar nebula}",
  journal = {\mnras},
 keywords = {ASTRONOMICAL MODELS, INTERPLANETARY MEDIUM, PROTOPLANETS, STELLAR MASS ACCRETION, SUN, CONVECTION, PLANETARY EVOLUTION, PLANETARY MASS, SOLAR SYSTEM},
     year = 1980,
    month = apr,
   volume = 191,
    pages = {37-48},
   adsurl = {http://adsabs.harvard.edu/abs/1980MNRAS.191...37L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1983MNRAS.205..359F,
   author = {{Faulkner}, J. and {Lin}, D.~N.~C. and {Papaloizou}, J.},
    title = "{On the evolution of accretion disc flow in cataclysmic variables. I - The prospect of a limit cycle in dwarf nova systems}",
  journal = {\mnras},
 keywords = {ACCRETION DISKS, DWARF NOVAE, STELLAR MASS ACCRETION, STELLAR TEMPERATURE, VARIABLE STARS, OPACITY, STEADY STATE, STELLAR STRUCTURE, THERMODYNAMICS},
     year = 1983,
    month = oct,
   volume = 205,
    pages = {359-375},
   adsurl = {http://adsabs.harvard.edu/abs/1983MNRAS.205..359F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1986ApJ...309..275H,
   author = {{Hartmann}, L. and {Hewett}, R. and {Stahler}, S. and {Mathieu}, R.~D.
	},
    title = "{Rotational and radial velocities of T Tauri stars}",
  journal = {\apj},
 keywords = {ANGULAR MOMENTUM, PRE-MAIN SEQUENCE STARS, RADIAL VELOCITY, STELLAR EVOLUTION, STELLAR ROTATION, T TAURI STARS, GRAVITATIONAL COLLAPSE, H ALPHA LINE,
MOLECULAR CLOUDS, ORION NEBULA, TAURUS CONSTELLATION},
     year = 1986,
    month = oct,
   volume = 309,
    pages = {275-293},
      doi = {10.1086/164599},
   adsurl = {http://adsabs.harvard.edu/abs/1986ApJ...309..275H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1981ApJ...245..960V,
   author = {{Vogel}, S.~N. and {Kuhi}, L.~V.},
    title = "{Rotational velocities of pre-main-sequence stars}",
  journal = {\apj},
 keywords = {MAIN SEQUENCE STARS, RADIAL VELOCITY, STAR CLUSTERS, STELLAR EVOLUTION, STELLAR ROTATION, STELLAR SPECTRA, A STARS, ANGULAR MOMENTUM, B STARS, EMISSION
SPECTRA, FOURIER TRANSFORMATION, H ALPHA LINE, HERTZSPRUNG-RUSSELL DIAGRAM, K LINES, LINE SPECTRA, POWER SPECTRA, T TAURI STARS},
     year = 1981,
    month = may,
   volume = 245,
    pages = {960-976},
      doi = {10.1086/158872},
   adsurl = {http://adsabs.harvard.edu/abs/1981ApJ...245..960V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1995ApJ...442..337P,
   author = {{Popham}, R. and {Narayan}, R.},
    title = "{Accretion disk boundary layers in cataclysmic variables. 1: Optically thick boundary layers}",
  journal = {\apj},
 keywords = {ACCRETION DISKS, BLACK BODY RADIATION, BOUNDARY LAYERS, CATACLYSMIC VARIABLES, LUMINOSITY, MATHEMATICAL MODELS, OPTICAL THICKNESS, WHITE DWARF STARS, ANGULAR
MOMENTUM, ANGULAR VELOCITY, ENERGY DISTRIBUTION, MASS FLOW RATE, OPACITY, RADIATIVE TRANSFER},
     year = 1995,
    month = mar,
   volume = 442,
    pages = {337-357},
      doi = {10.1086/175444},
   adsurl = {http://adsabs.harvard.edu/abs/1995ApJ...442..337P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1973A&A....24..337S,
   author = {{Shakura}, N.~I. and {Sunyaev}, R.~A.},
    title = "{Black holes in binary systems. Observational appearance.}",
  journal = {\aap},
     year = 1973,
   volume = 24,
    pages = {337-355},
   adsurl = {http://adsabs.harvard.edu/abs/1973A%26A....24..337S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009A&A...500...53K,
   author = {{King}, A.},
    title = "{Accretion: the gold mine opens. Commentary on: Shakura N. I. and Sunyaev R. A., 1973, A{\&}A, 24, 337}",
  journal = {\aap},
     year = 2009,
    month = jun,
   volume = 500,
    pages = {53-54},
      doi = {10.1051/0004-6361/200912147},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...500...53K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1984ApJS...55..367C,
   author = {{Cannizzo}, J.~K. and {Wheeler}, J.~C.},
    title = "{The vertical structure and stability of alpha model accretion disks}",
  journal = {\apjs},
 keywords = {ACCRETION DISKS, BINARY STARS, STELLAR MASS ACCRETION, STELLAR STRUCTURE, VARIABLE STARS, X RAY SOURCES, CONVECTION, DWARF NOVAE, OPACITY, RADIATIVE
TRANSFER, STELLAR LUMINOSITY, STELLAR MODELS, THERMAL INSTABILITY},
     year = 1984,
    month = jul,
   volume = 55,
    pages = {367-388},
      doi = {10.1086/190959},
   adsurl = {http://adsabs.harvard.edu/abs/1984ApJS...55..367C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1993ApJ...416..679K,
   author = {{Kley}, W. and {Papaloizou}, J.~C.~B. and {Lin}, D.~N.~C.},
    title = "{On the Angular Momentum Transport Associated with Convective Eddies in Accretion Disks}",
  journal = {\apj},
 keywords = {ACCRETION, ACCRETION DISKS, CONVECTION, HYDRODYNAMICS, STARS: FORMATION},
     year = 1993,
    month = oct,
   volume = 416,
    pages = {679},
      doi = {10.1086/173268},
   adsurl = {http://adsabs.harvard.edu/abs/1993ApJ...416..679K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1992ApJS...80..753S,
   author = {{Stone}, J.~M. and {Norman}, M.~L.},
    title = "{ZEUS-2D: A radiation magnetohydrodynamics code for astrophysical flows in two space dimensions. I - The hydrodynamic algorithms and tests.}",
  journal = {\apjs},
 keywords = {COMPUTATIONAL ASTROPHYSICS, COSMIC PLASMA, HYDRODYNAMIC EQUATIONS, MAGNETOHYDRODYNAMIC FLOW, SELF CONSISTENT FIELDS, COMPUTATIONAL GRIDS, FINITE DIFFERENCE
THEORY, PLASMA RADIATION, POISSON EQUATION, RADIATIVE TRANSFER},
     year = 1992,
    month = jun,
   volume = 80,
    pages = {753-790},
      doi = {10.1086/191680},
   adsurl = {http://adsabs.harvard.edu/abs/1992ApJS...80..753S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{Press:2007:NRE:1403886,
 author = {Press, William H. and Teukolsky, Saul A. and Vetterling, William T. and Flannery, Brian P.},
 title = {Numerical Recipes 3rd Edition: The Art of Scientific Computing},
 year = {2007},
 isbn = {0521880688, 9780521880688},
 edition = {3},
 publisher = {Cambridge University Press},
 address = {New York, NY, USA},
}

@BOOK{2005mmp..book.....A,
   author = {{Arfken}, G.~B. and {Weber}, H.~J.},
    title = "{Mathematical methods for physicists 6th ed.}",
     year = 2005,
   adsurl = {http://adsabs.harvard.edu/abs/2005mmp..book.....A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System},
publisher = {Academic Press}
}

booktitle = {''Mathematical methods for physicists 6th ed.by George B.~Arfken and Hans J.~Weber.~Published :Amsterdam; Boston : Elsevier, c2005.~xii, 1182 p.~: ill.~; 25
cm.~ Includes bibliographical references and index.~ISBN :},

@BOOK{1973grav.book.....M,
   author = {{Misner}, C.~W. and {Thorne}, K.~S. and {Wheeler}, J.~A.},
    title = "{Gravitation}",
     year = 1973,
   adsurl = {http://adsabs.harvard.edu/abs/1973grav.book.....M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System},
publisher = {W.H.~Freeman and Co., San Francisco}
}


@BOOK{2006mmpe.book.....R,
   author = {{Riley}, K.~F. and {Hobson}, M.~P. and {Bence}, S.~J.},
    title = "{Mathematical Methods for Physics and Engineering - 3rd Edition}",
     year = 2006,
    month = mar,
      doi = {10.2277/0521861535},
   adsurl = {http://adsabs.harvard.edu/abs/2006mmpe.book.....R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System},
publisher = {Cambridge University Press}
}

%booktitle = {Mathematical Methods for Physics and Engineering - 3rd Edition, by K.~F.~Riley, M.~P.~Hobson and S.~J.~Bence, pp.~1362.~Cambridge University Press, March
%2006.~ISBN-10: 0521861535.~ISBN-13: 9780521861533},

@BOOK{1984oup..book.....M,
   author = {{Mihalas}, D. and {Mihalas}, B.~W.},
    title = "{Foundations of radiation hydrodynamics}",
 keywords = {ASTROPHYSICS, COMPRESSIBLE FLUIDS, GAS DYNAMICS, HYDRODYNAMIC EQUATIONS, RADIATION LAWS, RADIATIVE HEAT TRANSFER, EQUATIONS OF MOTION, GRAVITATIONAL WAVES,
IDEAL FLUIDS, KINEMATICS, RADIATION DISTRIBUTION, RELATIVITY, SHOCK WAVES, SOUND WAVES, STATISTICAL MECHANICS, TENSOR ANALYSIS, THERMAL RADIATION, THERMODYNAMICS, VISCOUS
FLUIDS, WIND (METEOROLOGY)},
     year = 1984,
   adsurl = {http://adsabs.harvard.edu/abs/1984oup..book.....M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System},
publisher = {Oxford University Press, New York}
}

%booktitle = {New York, Oxford University Press, 1984, 731 p.},

@BOOK{1992aae..book.....M,
   author = {{Maran}, S.~P.},
    title = "{The astronomy and astrophysics encyclopedia}",
 keywords = {DICTIONARIES, ASTRONOMY, ASTROPHYSICS},
     year = 1992,
   adsurl = {http://adsabs.harvard.edu/abs/1992aae..book.....M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System},
publisher = {Cambridge University Press}
}

%booktitle = {New York: Van Nostrand Reinhold, and Cambridge: Cambridge University Press, 1992, edited by Maran, Stephen P.},

@BOOK{1985ibs..book.....P,
   author = {{Pringle}, J.~E. and {Wade}, R.~A.},
    title = "{Interacting binary stars}",
 keywords = {INTERACTING BINARY STARS, X RAY BINARY STARS, CONTACT BINARY STARS, CATACLYSMIC VARIABLE STARS},
     year = 1985,
   adsurl = {http://adsabs.harvard.edu/abs/1985ibs..book.....P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System},
publisher = {Cambridge University Press}
}

booktitle = {Interacting Binary Stars},

@ARTICLE{1982SSRv...32..379V,
   author = {{Verbunt}, F.},
    title = "{Accretion disks in stellar X-ray sources - A review of the basic theory of accretion disks and its problems}",
  journal = {\ssr},
 keywords = {ACCRETION DISKS, BINARY STARS, MILKY WAY GALAXY, STELLAR MODELS, X RAY SOURCES, BLACK HOLES (ASTRONOMY), EQUATIONS OF STATE, GAS STREAMS, HYDRODYNAMIC
EQUATIONS, MASS TRANSFER, NEUTRON STARS, VISCOSITY, WHITE DWARF STARS},
     year = 1982,
   volume = 32,
    pages = {379-404},
      doi = {10.1007/BF00177448},
   adsurl = {http://adsabs.harvard.edu/abs/1982SSRv...32..379V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1999AstL...25..269I,
   author = {{Inogamov}, N.~A. and {Sunyaev}, R.~A.},
    title = "{Spread of matter over a neutron-star surface during disk accretion}",
  journal = {Ast.~Lett.},
   eprint = {arXiv:astro-ph/9904333},
     year = 1999,
    month = may,
   volume = 25,
    pages = {269-293},
   adsurl = {http://adsabs.harvard.edu/abs/1999AstL...25..269I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1981ARA&A..19..137P,
   author = {{Pringle}, J.~E.},
    title = "{Accretion discs in astrophysics}",
  journal = {\araa},
 keywords = {ASTROPHYSICS, DISKS (SHAPES), GRAVITATIONAL EFFECTS, MASS TRANSFER, RADIATIVE TRANSFER, STELLAR MASS ACCRETION, ANGULAR MOMENTUM, CIRCULAR ORBITS, NEUTRON
STARS, ORBITAL MECHANICS, ROTATING FLUIDS, STELLAR RADIATION, VISCOSITY},
     year = 1981,
   volume = 19,
    pages = {137-162},
      doi = {10.1146/annurev.aa.19.090181.001033},
   adsurl = {http://adsabs.harvard.edu/abs/1981ARA%26A..19..137P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@UNPUBLISHED{Werner,
	author = {{Werner}, Klaus},
	title  = "{Einführung in die Astronomie und Astrophysik}",
	note   = "{Vorlesungsskript}",
	year   = 2012
}

@UNPUBLISHED{Kley,
	author = {{Kley}, Wilhelm},
	title  = "{Theoretische Astrophysik}",
	note   = "{Vorlesungsskript}",
	year   = 2012
}

@ARTICLE{2003A&A...399..395S,
   author = {{Speith}, R. and {Kley}, W.},
    title = "{Stability of the viscously spreading ring}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0212139},
 keywords = {accretion, accretion discs, hydrodynamics, methods: numerical},
     year = 2003,
    month = feb,
   volume = 399,
    pages = {395-407},
      doi = {10.1051/0004-6361:20021783},
   adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...399..395S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1992ApJ...401..317L,
   author = {{Lubow}, S.~H.},
    title = "{Dynamics of eccentric disks with application to superhump binaries}",
  journal = {\apj},
 keywords = {ACCRETION DISKS, BINARY STARS, CATACLYSMIC VARIABLES, PLANETARY RINGS, STELLAR ORBITS, COUPLED MODES, ECCENTRIC ORBITS, ECCENTRICITY, NOVAE, ORBITAL
RESONANCES (CELESTIAL MECHANICS), PRECESSION},
     year = 1992,
    month = dec,
   volume = 401,
    pages = {317-324},
      doi = {10.1086/172062},
   adsurl = {http://adsabs.harvard.edu/abs/1992ApJ...401..317L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1991ApJ...381..268L,
   author = {{Lubow}, S.~H.},
    title = "{Simulations of tidally driven eccentric instabilities with application to superhumps}",
  journal = {\apj},
 keywords = {BINARY STARS, ORBITAL RESONANCES (CELESTIAL MECHANICS), SHELL STARS, STELLAR MODELS, STELLAR STRUCTURE, COMPUTATIONAL ASTROPHYSICS, DIGITAL SIMULATION,
ECCENTRIC ORBITS, STELLAR ENVELOPES, SYSTEMS STABILITY, TIDES},
     year = 1991,
    month = nov,
   volume = 381,
    pages = {268-277},
      doi = {10.1086/170648},
   adsurl = {http://adsabs.harvard.edu/abs/1991ApJ...381..268L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008A&A...487..671K,
   author = {{Kley}, W. and {Papaloizou}, J.~C.~B. and {Ogilvie}, G.~I.},
    title = "{Simulations of eccentric disks in close binary systems}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0806.3873},
 keywords = {accretion, accretion disks, stars: binaries: close, novae, cataclysmic variables},
     year = 2008,
    month = aug,
   volume = 487,
    pages = {671-687},
      doi = {10.1051/0004-6361:200809953},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...487..671K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1989PASJ...41.1005O,
   author = {{Osaki}, Y.},
    title = "{A model for the superoutburst phenomenon of SU Ursae Majoris stars}",
  journal = {\pasj},
 keywords = {ACCRETION DISKS, DWARF NOVAE, STELLAR MODELS, STELLAR STRUCTURE, THERMAL INSTABILITY, ANGULAR MOMENTUM, ASTRONOMICAL PHOTOMETRY, BURSTS, MASS TRANSFER},
     year = 1989,
   volume = 41,
    pages = {1005-1033},
   adsurl = {http://adsabs.harvard.edu/abs/1989PASJ...41.1005O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1998MNRAS.297..323M,
   author = {{Murray}, J.~R.},
    title = "{Simulations of superhumps and superoutbursts}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/9710233},
 keywords = {ACCRETION, ACCRETION DISCS, HYDRODYNAMICS, INSTABILITIES, METHODS: NUMERICAL, BINARIES: CLOSE, NOVAE, CATACLYSMIC VARIABLES},
     year = 1998,
    month = jun,
   volume = 297,
    pages = {323-333},
      doi = {10.1046/j.1365-8711.1998.01504.x},
   adsurl = {http://adsabs.harvard.edu/abs/1998MNRAS.297..323M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1995CAS....28.....W,
   author = {{Warner}, B.},
    title = "{Cataclysmic variable stars.}",
  journal = {Cambridge Astrophysics Series},
 keywords = {Cataclysmic Binaries: Multiwavelength Observations, Cataclysmic Binaries: Models},
     year = 1995,
   volume = 28,
   adsurl = {http://adsabs.harvard.edu/abs/1995CAS....28.....W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{giovannelli1985multifrequency,
  title={Multifrequency Behavior of Galactic Accreting Sources},
  author={Giovannelli, F.},
  series={Frascati Workshop},
  url={http://books.google.de/books?id=vm0HNQAACAAJ},
  year={1985},
  publisher={Edizioni Scientifiche Siderea}
}

@ARTICLE{1998A&AS..129...83R,
   author = {{Ritter}, H. and {Kolb}, U.},
    title = "{Catalogue of cataclysmic binaries, low-mass X-ray binaries and related objects (Sixth edition)}",
  journal = {\aaps},
 keywords = {CATALOGS, NOVAE, CATACLYSMIC VARIABLES, BINARIES: CLOSE, X-RAYS: STARS},
     year = 1998,
    month = apr,
   volume = 129,
    pages = {83-85},
      doi = {10.1051/aas:1998175},
   adsurl = {http://adsabs.harvard.edu/abs/1998A%26AS..129...83R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{maran1992astronomy,
  title={The Astronomy and Astrophysics Encyclopedia},
  author={Maran, S.P.},
  isbn={9780521417440},
  lccn={lc91023241},
  url={http://books.google.de/books?id=hw36JwAACAAJ},
  year={1992},
  publisher={Cambridge University Press}
}

@PROCEEDINGS{1991foap.conf.....G,
    title = "{Frontier objects in astrophysics and particle physics. Proceedings.}",
     year = 1991,
   editor = {{Giovannelli}, F. and {Mannocchi}, G.},
   adsurl = {http://adsabs.harvard.edu/abs/1991foap.conf.....G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

booktitle = {Frontier Objects in Astrophysics and Particle Physics},

@ARTICLE{2000NewAR..44...75W,
   author = {{Wynn}, G.~A.},
    title = "{Accretion flows in magnetic CVs}",
  journal = {\nar},
     year = 2000,
    month = apr,
   volume = 44,
    pages = {75-80},
      doi = {10.1016/S1387-6473(00)00017-8},
   adsurl = {http://adsabs.harvard.edu/abs/2000NewAR..44...75W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1984ApJS...54..443P,
   author = {{Patterson}, J.},
    title = "{The evolution of cataclysmic and low-mass X-ray binaries}",
  journal = {\apjs},
 keywords = {BINARY STARS, STELLAR EVOLUTION, STELLAR MASS EJECTION, X RAY BINARIES, X RAY SOURCES, X RAY STARS, ACCRETION DISKS, ANGULAR MOMENTUM, DWARF NOVAE, ORBITAL
		ELEMENTS, STAR DISTRIBUTION, STELLAR MAGNETIC FIELDS, STELLAR ROTATION, STELLAR STRUCTURE, STELLAR WINDS, VARIABLE STARS, WHITE DWARF STARS},
     year = 1984,
    month = apr,
   volume = 54,
    pages = {443-493},
      doi = {10.1086/190940},
   adsurl = {http://adsabs.harvard.edu/abs/1984ApJS...54..443P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1987MNRAS.227...23W,
   author = {{Warner}, B.},
    title = "{Absolute magnitudes of cataclysmic variables}",
  journal = {\mnras},
 keywords = {ACCRETION DISKS, CATACLYSMIC VARIABLES, COMPUTATIONAL ASTROPHYSICS, DWARF NOVAE, STELLAR MAGNITUDE, MASS TO LIGHT RATIOS, MASS TRANSFER, ORBITAL ELEMENTS,
STELLAR EVOLUTION},
     year = 1987,
    month = jul,
   volume = 227,
    pages = {23-73},
   adsurl = {http://adsabs.harvard.edu/abs/1987MNRAS.227...23W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1999MmSAI..70..987G,
   author = {{Giovannelli}, F. and {Sabau-Graziati}, L.},
    title = "{SS Cygni: a frontier system between intermediate polars and non-magnetic cataclysmic variables.}",
  journal = {\memsai},
 keywords = {Cataclysmic Binaries: Polars, Cataclysmic Binaries: Classification, Cataclysmic Binaries: Models},
     year = 1999,
   volume = 70,
    pages = {987-1003},
   adsurl = {http://adsabs.harvard.edu/abs/1999MmSAI..70..987G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{RG2003,
	author = {{Rodriguez-Gil}, P.},
	title  = "{PhD-Thesis}",
	publisher= {La Laguna Universität, Spanien},
	year   = 2003,
	moth   = feb
}

@ARTICLE{1968MNRAS.138..359M,
   author = {{Mestel}, L.},
    title = "{Magnetic braking by a stellar wind-I}",
  journal = {\mnras},
     year = 1968,
   volume = 138,
    pages = {359},
   adsurl = {http://adsabs.harvard.edu/abs/1968MNRAS.138..359M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004PASP..116..115W,
   author = {{Warner}, B.},
    title = "{Rapid Oscillations in Cataclysmic Variables}",
  journal = {\pasp},
   eprint = {arXiv:astro-ph/0312182},
 keywords = {Stars: Novae, Cataclysmic Variables, stars: binaries: close},
     year = 2004,
    month = feb,
   volume = 116,
    pages = {115-132},
      doi = {10.1086/381742},
   adsurl = {http://adsabs.harvard.edu/abs/2004PASP..116..115W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2005ASPC..330..227W,
   author = {{Warner}, B. and {Woudt}, P.~A.},
    title = "{DNOs and QPOs in Cataclysmic Variables}",
booktitle = {The Astrophysics of Cataclysmic Variables and Related Objects},
     year = 2005,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 330,
   eprint = {arXiv:astro-ph/0409287},
   editor = {{Hameury}, J.-M. and {Lasota}, J.-P.},
    month = aug,
    pages = {227},
   adsurl = {http://adsabs.harvard.edu/abs/2005ASPC..330..227W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006MNRAS.368..361P,
   author = {{Pretorius}, M.~L. and {Warner}, B. and {Woudt}, P.~A.},
    title = "{Dwarf nova oscillations and quasi-periodic oscillations in cataclysmic variables - V. Results from an extensive survey}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/0601539},
 keywords = {accretion, accretion discs, stars: dwarf novae, novae, cataclysmic variables, stars: oscillations},
     year = 2006,
    month = may,
   volume = 368,
    pages = {361-370},
      doi = {10.1111/j.1365-2966.2006.10123.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.368..361P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1986PASP...98..821S,
   author = {{Sion}, E.~M.},
    title = "{Recent advances on the formation and evolution of white dwarfs}",
  journal = {\pasp},
 keywords = {STAR FORMATION, STELLAR EVOLUTION, STELLAR SPECTRA, WHITE DWARF STARS, CATACLYSMIC VARIABLES, STELLAR COMPOSITION, STELLAR ENVELOPES, STELLAR MASS ACCRETION,
X RAY STARS},
     year = 1986,
    month = sep,
   volume = 98,
    pages = {821-837},
      doi = {10.1086/131831},
   adsurl = {http://adsabs.harvard.edu/abs/1986PASP...98..821S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1991AJ....102..295S,
   author = {{Sion}, E.~M.},
    title = "{Cataclysmic variable evolution - Clues from the underlying white dwarf}",
  journal = {\aj},
 keywords = {CATACLYSMIC VARIABLES, MAGNETIC STARS, STELLAR EVOLUTION, WHITE DWARF STARS, NOVAE, STELLAR ENVELOPES, STELLAR LUMINOSITY, STELLAR MASS, STELLAR ORBITS,
STELLAR TEMPERATURE},
     year = 1991,
    month = jul,
   volume = 102,
    pages = {295-302},
      doi = {10.1086/115877},
   adsurl = {http://adsabs.harvard.edu/abs/1991AJ....102..295S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1998ESASP.413..381S,
   author = {{Szkody}, P.},
    title = "{UV Spectra of Dwarf Novae: a Window to the White Dwarf and the Accretion Process}",
booktitle = {Ultraviolet Astrophysics Beyond the IUE Final Archive},
     year = 1998,
   series = {ESA Special Publication},
   volume = 413,
   editor = {{Wamsteker}, W. and {Gonzalez Riestra}, R. and {Harris}, B.},
    pages = {381},
   adsurl = {http://adsabs.harvard.edu/abs/1998ESASP.413..381S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1981A&A...104L..10M,
   author = {{Meyer}, F. and {Meyer-Hofmeister}, E.},
    title = "{On the Elusive Cause of Cataclysmic Variable Outbursts}",
  journal = {\aap},
     year = 1981,
   volume = 104,
    pages = {L10},
   adsurl = {http://adsabs.harvard.edu/abs/1981A%26A...104L..10M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1982A&A...106...34M,
   author = {{Meyer}, F. and {Meyer-Hofmeister}, E.},
    title = "{Vertical structure of accretion disks}",
  journal = {\aap},
 keywords = {CONVECTION, ENERGY TRANSFER, NEUTRON STARS, RADIATIVE TRANSFER, STELLAR MASS ACCRETION, VARIABLE STARS, DISKS (SHAPES), ECLIPSING BINARY STARS, VERTICAL
ORIENTATION, X RAY BINARIES, X RAY IRRADIATION, X RAY SOURCES},
     year = 1982,
    month = feb,
   volume = 106,
    pages = {34-42},
   adsurl = {http://adsabs.harvard.edu/abs/1982A%26A...106...34M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1983A&A...128..420M,
   author = {{Meyer}, F. and {Meyer-Hofmeister}, E.},
    title = "{Accretion disks in cataclysmic variables - The influence of the frictional parameter alpha on the structure}",
  journal = {\aap},
 keywords = {ACCRETION DISKS, BINARY STARS, STELLAR MASS ACCRETION, VARIABLE STARS, DWARF NOVAE, FLUX DENSITY, FRICTION, STELLAR MAGNETIC FIELDS, VISCOSITY},
     year = 1983,
    month = dec,
   volume = 128,
    pages = {420-425},
   adsurl = {http://adsabs.harvard.edu/abs/1983A%26A...128..420M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1984AcA....34..161S,
   author = {{Smak}, J.},
    title = "{Accretion in cataclysmic binaries. IV - Accretion disks in dwarf novae}",
  journal = {\actaa},
 keywords = {ACCRETION DISKS, CATACLYSMIC VARIABLES, DWARF NOVAE, STELLAR MASS ACCRETION, STELLAR MODELS, BINARY STARS, LIGHT CURVE, STELLAR FLARES, STELLAR STRUCTURE,
STELLAR TEMPERATURE, THERMAL INSTABILITY, VISCOSITY},
     year = 1984,
   volume = 34,
    pages = {161-189},
   adsurl = {http://adsabs.harvard.edu/abs/1984AcA....34..161S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1984PASP...96....5S,
   author = {{Smak}, J.},
    title = "{Outbursts of dwarf novae}",
  journal = {\pasp},
 keywords = {ACCRETION DISKS, BURSTS, DWARF NOVAE, STELLAR RADIATION, VARIABLE STARS, BINARY STARS, LIGHT CURVE, STELLAR MASS EJECTION, STELLAR MODELS, VISCOSITY},
     year = 1984,
    month = jan,
   volume = 96,
    pages = {5-18},
      doi = {10.1086/131295},
   adsurl = {http://adsabs.harvard.edu/abs/1984PASP...96....5S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002MmSAI..73..206S,
   author = {{Smak}, J.},
    title = "{Cataclysmic variables and viscosity of their accretion disks.}",
  journal = {\memsai},
     year = 2002,
   volume = 73,
    pages = {206-212},
   adsurl = {http://adsabs.harvard.edu/abs/2002MmSAI..73..206S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003ApJ...586.1297S,
   author = {{Sano}, T. and {Stone}, J.~M.},
    title = "{A Local One-Zone Model of MagnetoHydroDynamic Turbulence in Dwarf Nova Disks}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0212076},
 keywords = {Accretion, Accretion Disks, Diffusion, Instabilities, Magnetohydrodynamics: MHD, Stars: Novae, Cataclysmic Variables, Turbulence},
     year = 2003,
    month = apr,
   volume = 586,
    pages = {1297-1304},
      doi = {10.1086/367723},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...586.1297S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1999AcA....49..391S,
   author = {{Smak}, J.},
    title = "{Dwarf Nova Outbursts. III. The Viscosity Parameter alpha}",
  journal = {\actaa},
 keywords = {ACCRETION: ACCRETION DISKS, BINARIES: CLOSE, NOVAE: CATACLYSMIC VARIABLES},
     year = 1999,
    month = sep,
   volume = 49,
    pages = {391-401},
   adsurl = {http://adsabs.harvard.edu/abs/1999AcA....49..391S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1994ApJ...435..389C,
   author = {{Cannizzo}, J.~K.},
    title = "{On the decay of outbursts in dwarf novae and X-ray novae}",
  journal = {\apj},
 keywords = {ACCRETION DISKS, CATACLYSMIC VARIABLES, DWARF NOVAE, STELLAR MASS ACCRETION, STELLAR MASS EJECTION, STELLAR MODELS, MATHEMATICAL MODELS, TIME DEPENDENCE},
     year = 1994,
    month = nov,
   volume = 435,
    pages = {389-397},
      doi = {10.1086/174821},
   adsurl = {http://adsabs.harvard.edu/abs/1994ApJ...435..389C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1989ApJ...341..974W,
   author = {{Wood}, J.~H. and {Horne}, K. and {Berriman}, G. and {Wade}, R.~A.
	},
    title = "{Eclipse studies of the dwarf nova OY Carinae in quiescence}",
  journal = {\apj},
 keywords = {DWARF NOVAE, ECLIPSING BINARY STARS, LIGHT CURVE, STELLAR SPECTROPHOTOMETRY, RED DWARF STARS, STELLAR MODELS, STELLAR ORBITS, WHITE DWARF STARS},
     year = 1989,
    month = jun,
   volume = 341,
    pages = {974-996},
      doi = {10.1086/167557},
   adsurl = {http://adsabs.harvard.edu/abs/1989ApJ...341..974W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1994tad..conf...77H,
   author = {{Horne}, K.},
    title = "{Accretion disks in cataclysmic variable stars: Recent observational developments}",
booktitle = {NATO ASIC Proc. 417: Theory of Accretion Disks - 2},
     year = 1994,
   editor = {{Duschl}, W.~J. and {Frank}, J. and {Meyer}, F. and {Meyer-Hofmeister}, E. and 
	{Tscharnuter}, W.~M.},
    pages = {77},
   adsurl = {http://adsabs.harvard.edu/abs/1994tad..conf...77H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1991ApJ...372..659M,
   author = {{Mauche}, C.~W. and {Wade}, R.~A. and {Polidan}, R.~S. and {van der Woerd}, H. and 
	{Paerels}, F.~B.~S.},
    title = "{On the X-ray emitting boundary layer of the dwarf nova VW Hydri}",
  journal = {\apj},
 keywords = {DWARF NOVAE, STELLAR SPECTROPHOTOMETRY, ULTRAVIOLET PHOTOMETRY, X RAY SOURCES, ACCRETION DISKS, EXOSAT SATELLITE, HYDROGEN ATOMS, STELLAR LUMINOSITY, STELLAR
TEMPERATURE},
     year = 1991,
    month = may,
   volume = 372,
    pages = {659-663},
      doi = {10.1086/170008},
   adsurl = {http://adsabs.harvard.edu/abs/1991ApJ...372..659M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1991A&A...246L..44B,
   author = {{Belloni}, T. and {Verbunt}, F. and {Beuermann}, K. and {Bunk}, W. and 
	{Izzo}, C. and {Kley}, W. and {Pietsch}, W. and {Ritter}, H. and 
	{Thomas}, H.~C. and {Voges}, W.},
    title = "{ROSAT observation of the boundary layer between the white dwarf and the accretion disk of VW Hydri}",
  journal = {\aap},
 keywords = {ACCRETION DISKS, CATACLYSMIC VARIABLES, DWARF NOVAE, ROSAT MISSION, WHITE DWARF STARS, X RAY SPECTRA, PROPORTIONAL COUNTERS, RADIANT FLUX DENSITY, SKY
SURVEYS (ASTRONOMY)},
     year = 1991,
    month = jun,
   volume = 246,
    pages = {L44-L46},
   adsurl = {http://adsabs.harvard.edu/abs/1991A%26A...246L..44B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1994ApJ...430L..53S,
   author = {{Sion}, E.~M. and {Long}, K.~S. and {Szkody}, P. and {Huang}, M.
	},
    title = "{Hubble space telescope Goddard High-Resolution Spectrograph observation of U Geminorum during quiescence: Evidence for a slowly rotating white dwarf}",
  journal = {\apjl},
 keywords = {SPECTRUM ANALYSIS, STELLAR ROTATION, ULTRAVIOLET SPECTROMETERS, WHITE DWARF STARS, ANGULAR VELOCITY, HUBBLE SPACE TELESCOPE, LINE SHAPE, RED SHIFT},
     year = 1994,
    month = jul,
   volume = 430,
    pages = {L53-L56},
      doi = {10.1086/187436},
   adsurl = {http://adsabs.harvard.edu/abs/1994ApJ...430L..53S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1990LNP...369..228D,
   author = {{Drew}, J.~E.},
    title = "{Winds from Disks}",
booktitle = {IAU Colloq. 122: Physics of Classical Novae},
     year = 1990,
   series = {Lecture Notes in Physics, Berlin Springer Verlag},
   volume = 369,
   editor = {{Cassatella}, A. and {Viotti}, R.},
    pages = {228},
      doi = {10.1007/3-540-53500-4_130},
   adsurl = {http://adsabs.harvard.edu/abs/1990LNP...369..228D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1992MNRAS.255..237W,
   author = {{Woods}, J.~A. and {Verbunt}, F. and {Collier Cameron}, A. and 
	{Drew}, J.~E. and {Piters}, A.},
    title = "{Time dependence of the UV resonance lines in the cataclysmic variables YZ Cnc, IR GEM and V3885 SGR}",
  journal = {\mnras},
 keywords = {CATACLYSMIC VARIABLES, RESONANCE LINES, STELLAR SPECTROPHOTOMETRY, ULTRAVIOLET SPECTRA, ABSORPTION SPECTRA, EMISSION SPECTRA, IUE, LINE SPECTRA, STELLAR
MAGNITUDE, TIME DEPENDENCE},
     year = 1992,
    month = mar,
   volume = 255,
    pages = {237-242},
   adsurl = {http://adsabs.harvard.edu/abs/1992MNRAS.255..237W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1931ApJ....74...81C,
   author = {{Chandrasekhar}, S.},
    title = "{The Maximum Mass of Ideal White Dwarfs}",
  journal = {\apj},
     year = 1931,
    month = jul,
   volume = 74,
    pages = {81},
      doi = {10.1086/143324},
   adsurl = {http://adsabs.harvard.edu/abs/1931ApJ....74...81C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1995ASPC...72..105L,
   author = {{Livio}, M.},
    title = "{On the Fate of Accreting White Dwarfs in Cataclysmic Variables and Related Systems}",
booktitle = {Millisecond Pulsars.  A Decade of Surprise},
     year = 1995,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 72,
   editor = {{Fruchter}, A.~S. and {Tavani}, M. and {Backer}, D.~C.},
    pages = {105},
   adsurl = {http://adsabs.harvard.edu/abs/1995ASPC...72..105L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1948ZNatA...3..524W,
   author = {{Weizs{\"a}cker}, C.~F.~V.},
    title = "{Die Rotation kosmischer Gasmassen}",
  journal = {Zeitschrift Naturforschung Teil A},
     year = 1948,
   volume = 3,
    pages = {524},
   adsurl = {http://adsabs.harvard.edu/abs/1948ZNatA...3..524W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{jeffreys1924earth,
  title={The earth: its origin, history and physical constitution},
  author={Jeffreys, H.},
  lccn={25000340},
  url={http://books.google.de/books?id=j71NAAAAMAAJ},
  year={1924},
  publisher={University Press}
}

@BOOK{1969QB981.S26......,
   author = {{Safronov}, V.~S.},
    title = "{Evoliutsiia doplanetnogo oblaka.}",
 keywords = {COSMOGONY, COSMOLOGY, EARTH, PLANETS},
     year = 1969,
   adsurl = {http://adsabs.harvard.edu/abs/1969QB981.S26......},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System},
publisher = {Nauka, Moskva}
}

booktitle = {1969.},

@ARTICLE{1971AZh....48..881B,
   author = {{Bisnovatyi-Kogan}, G.~S. and {Syunyaev}, R.~A.},
    title = "{Galaxy Nuclei and Quasars as Infrared Emission Sources.}",
  journal = {\azh},
     year = 1971,
    month = oct,
   volume = 48,
    pages = {881},
   adsurl = {http://adsabs.harvard.edu/abs/1971AZh....48..881B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1971AZh....48..479S,
   author = {{Shvartsman}, V.~F.},
    title = "{Halos around ''Black Holes''.}",
  journal = {\azh},
     year = 1971,
    month = jun,
   volume = 48,
    pages = {479},
   adsurl = {http://adsabs.harvard.edu/abs/1971AZh....48..479S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1946ApNr....4....1W,
   author = {{Wasiutynski}, J.},
    title = "{Studies in Hydrodynamics and Structure of Stars and Planets}",
  journal = {Astrophysica Norvegica},
     year = 1946,
   volume = 4,
    pages = {1-497},
   adsurl = {http://adsabs.harvard.edu/abs/1946ApNr....4....1W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1936RSPSA.157..546T,
   author = {{Taylor}, G.~I.},
    title = "{Fluid Friction between Rotating Cylinders. I. Torque Measurements}",
  journal = {Proc.~R.~Soc.~A},
     year = 1936,
    month = dec,
   volume = 157,
    pages = {546-564},
      doi = {10.1098/rspa.1936.0215},
   adsurl = {http://adsabs.harvard.edu/abs/1936RSPSA.157..546T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005ApJ...629..383M,
   author = {{Mukhopadhyay}, B. and {Afshordi}, N. and {Narayan}, R.},
    title = "{Bypass to Turbulence in Hydrodynamic Accretion Disks: An Eigenvalue Approach}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0412193},
 keywords = {Accretion, Accretion Disks, Hydrodynamics, Instabilities, Turbulence},
     year = 2005,
    month = aug,
   volume = 629,
    pages = {383-396},
      doi = {10.1086/431419},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...629..383M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005ApJ...629..373A,
   author = {{Afshordi}, N. and {Mukhopadhyay}, B. and {Narayan}, R.},
    title = "{Bypass to Turbulence in Hydrodynamic Accretion: Lagrangian Analysis of Energy Growth}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0412194},
 keywords = {Accretion, Accretion Disks, Hydrodynamics, Instabilities, Turbulence},
     year = 2005,
    month = aug,
   volume = 629,
    pages = {373-382},
      doi = {10.1086/431418},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...629..373A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1992ApJ...388..438R,
   author = {{Ryu}, D. and {Goodman}, J.},
    title = "{Convective instability in differentially rotating disks}",
  journal = {\apj},
 keywords = {ACCRETION DISKS, CONVECTIVE FLOW, MAGNETOHYDRODYNAMIC STABILITY, MASS FLOW, ROTATING PLASMAS, ACTIVE GALACTIC NUCLEI, ANGULAR MOMENTUM, ANGULAR VELOCITY,
MOMENTUM TRANSFER, QUASARS},
     year = 1992,
    month = apr,
   volume = 388,
    pages = {438-450},
      doi = {10.1086/171165},
   adsurl = {http://adsabs.harvard.edu/abs/1992ApJ...388..438R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006ApJ...652.1020B,
   author = {{Balbus}, S.~A. and {Hawley}, J.~F.},
    title = "{An Exact, Three-dimensional, Time-dependent Wave Solution in Local Keplerian Flow}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0608429},
 keywords = {Accretion, Accretion Disks, Galaxies: Magnetic Fields, Instabilities, Magnetic Fields, Magnetohydrodynamics: MHD},
     year = 2006,
    month = dec,
   volume = 652,
    pages = {1020-1027},
      doi = {10.1086/508320},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...652.1020B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1996ApJ...467...76B,
   author = {{Balbus}, S.~A. and {Hawley}, J.~F. and {Stone}, J.~M.},
    title = "{Nonlinear Stability, Hydrodynamical Turbulence, and Transport in Disks}",
  journal = {\apj},
 keywords = {ACCRETION, ACCRETION DISKS, HYDRODYNAMICS, INSTABILITIES, METHODS: NUMERICAL, TURBULENCE},
     year = 1996,
    month = aug,
   volume = 467,
    pages = {76},
      doi = {10.1086/177585},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...467...76B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1996ApJ...464..364S,
   author = {{Stone}, J.~M. and {Balbus}, S.~A.},
    title = "{Angular Momentum Transport in Accretion Disks via Convection}",
  journal = {\apj},
 keywords = {ACCRETION, ACCRETION DISKS, CONVECTION, HYDRODYNAMICS, INSTABILITIES},
     year = 1996,
    month = jun,
   volume = 464,
    pages = {364},
      doi = {10.1086/177328},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...464..364S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1997ASPC..121...90B,
   author = {{Balbus}, S.~A. and {Hawley}, J.~F.},
    title = "{Instability, Turbulence, and Enhanced Transport in Accretion Disks}",
booktitle = {IAU Colloq. 163: Accretion Phenomena and Related Outflows},
     year = 1997,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 121,
   editor = {{Wickramasinghe}, D.~T. and {Bicknell}, G.~V. and {Ferrario}, L.
	},
    pages = {90},
   adsurl = {http://adsabs.harvard.edu/abs/1997ASPC..121...90B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1999ApJ...518..394H,
   author = {{Hawley}, J.~F. and {Balbus}, S.~A. and {Winters}, W.~F.},
    title = "{Local Hydrodynamic Stability of Accretion Disks}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/9811057},
 keywords = {ACCRETION, ACCRETION DISKS, HYDRODYNAMICS, INSTABILITIES, STARS: PRE-MAIN-SEQUENCE},
     year = 1999,
    month = jun,
   volume = 518,
    pages = {394-404},
      doi = {10.1086/307282},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...518..394H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006Natur.444..343J,
   author = {{Ji}, H. and {Burin}, M. and {Schartman}, E. and {Goodman}, J.
	},
    title = "{Hydrodynamic turbulence cannot transport angular momentum effectively in astrophysical disks}",
  journal = {\nat},
   eprint = {arXiv:astro-ph/0611481},
     year = 2006,
    month = nov,
   volume = 444,
    pages = {343-346},
      doi = {10.1038/nature05323},
   adsurl = {http://adsabs.harvard.edu/abs/2006Natur.444..343J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1991ApJ...376..214B,
   author = {{Balbus}, S.~A. and {Hawley}, J.~F.},
    title = "{A powerful local shear instability in weakly magnetized disks. I - Linear analysis. II - Nonlinear evolution}",
  journal = {\apj},
 keywords = {ACCRETION DISKS, MAGNETOHYDRODYNAMIC STABILITY, STELLAR MAGNETIC FIELDS, STELLAR MASS ACCRETION, BOUSSINESQ APPROXIMATION, COMPUTATIONAL ASTROPHYSICS, LINEAR
SYSTEMS},
     year = 1991,
    month = jul,
   volume = 376,
    pages = {214-233},
      doi = {10.1086/170270},
   adsurl = {http://adsabs.harvard.edu/abs/1991ApJ...376..214B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003ARA&A..41..555B,
   author = {{Balbus}, S.~A.},
    title = "{Enhanced Angular Momentum Transport in Accretion Disks}",
  journal = {\araa},
   eprint = {arXiv:astro-ph/0306208},
     year = 2003,
   volume = 41,
    pages = {555-597},
      doi = {10.1146/annurev.astro.41.081401.155207},
   adsurl = {http://adsabs.harvard.edu/abs/2003ARA%26A..41..555B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1995ApJ...446..741B,
   author = {{Brandenburg}, A. and {Nordlund}, A. and {Stein}, R.~F. and 
	{Torkelsson}, U.},
    title = "{Dynamo-generated Turbulence and Large-Scale Magnetic Fields in a Keplerian Shear Flow}",
  journal = {\apj},
 keywords = {ACCRETION, ACCRETION DISKS, MAGNETOHYDRODYNAMICS: MHD, SHOCK WAVES, TURBULENCE},
     year = 1995,
    month = jun,
   volume = 446,
    pages = {741},
      doi = {10.1086/175831},
   adsurl = {http://adsabs.harvard.edu/abs/1995ApJ...446..741B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1995ApJ...440..742H,
   author = {{Hawley}, J.~F. and {Gammie}, C.~F. and {Balbus}, S.~A.},
    title = "{Local Three-dimensional Magnetohydrodynamic Simulations of Accretion Disks}",
  journal = {\apj},
 keywords = {ACCRETION, ACCRETION DISKS, INSTABILITIES, MAGNETOHYDRODYNAMICS: MHD},
     year = 1995,
    month = feb,
   volume = 440,
    pages = {742},
      doi = {10.1086/175311},
   adsurl = {http://adsabs.harvard.edu/abs/1995ApJ...440..742H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1996ApJ...464..690H,
   author = {{Hawley}, J.~F. and {Gammie}, C.~F. and {Balbus}, S.~A.},
    title = "{Local Three-dimensional Simulations of an Accretion Disk Hydromagnetic Dynamo}",
  journal = {\apj},
 keywords = {ACCRETION, ACCRETION DISKS, HYDRODYNAMICS, MAGNETOHYDRODYNAMICS: MHD, TURBULENCE},
     year = 1996,
    month = jun,
   volume = 464,
    pages = {690},
      doi = {10.1086/177356},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...464..690H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1996ApJ...463..656S,
   author = {{Stone}, J.~M. and {Hawley}, J.~F. and {Gammie}, C.~F. and {Balbus}, S.~A.
	},
    title = "{Three-dimensional Magnetohydrodynamical Simulations of Vertically Stratified Accretion Disks}",
  journal = {\apj},
 keywords = {ACCRETION, ACCRETION DISKS, INSTABILITIES, MAGNETOHYDRODYNAMICS: MHD, METHODS: NUMERICAL},
     year = 1996,
    month = jun,
   volume = 463,
    pages = {656},
      doi = {10.1086/177280},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...463..656S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001ApJ...550..824B,
   author = {{Brandenburg}, A.},
    title = "{The Inverse Cascade and Nonlinear Alpha-Effect in Simulations of Isotropic Helical Hydromagnetic Turbulence}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0006186},
 keywords = {Magnetohydrodynamics: MHD, Turbulence},
     year = 2001,
    month = apr,
   volume = 550,
    pages = {824-840},
      doi = {10.1086/319783},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...550..824B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004ApJ...605..321S,
   author = {{Sano}, T. and {Inutsuka}, S.-i. and {Turner}, N.~J. and {Stone}, J.~M.
	},
    title = "{Angular Momentum Transport by Magnetohydrodynamic Turbulence in Accretion Disks: Gas Pressure Dependence of the Saturation Level of the Magnetorotational
Instability}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0312480},
 keywords = {Accretion, Accretion Disks, Diffusion, Instabilities, Magnetohydrodynamics: MHD, Turbulence},
     year = 2004,
    month = apr,
   volume = 605,
    pages = {321-339},
      doi = {10.1086/382184},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...605..321S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1998ApJ...501L.189A,
   author = {{Armitage}, P.~J.},
    title = "{Turbulence and Angular Momentum Transport in Global Accretion Disk Simulation}",
  journal = {\apjl},
   eprint = {arXiv:astro-ph/9805133},
 keywords = {ACCRETION, ACCRETION DISKS, HYDRODYNAMICS, INSTABILITIES, MAGNETIC FIELDS, MAGNETOHYDRODYNAMICS: MHD, TURBULENCE},
     year = 1998,
    month = jul,
   volume = 501,
    pages = {L189},
      doi = {10.1086/311463},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...501L.189A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000ApJ...528..462H,
   author = {{Hawley}, J.~F.},
    title = "{Global Magnetohydrodynamical Simulations of Accretion Tori}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/9907385},
 keywords = {ACCRETION, ACCRETION DISKS, INSTABILITIES, MAGNETOHYDRODYNAMICS: MHD},
     year = 2000,
    month = jan,
   volume = 528,
    pages = {462-479},
      doi = {10.1086/308180},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...528..462H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001ApJ...554..534H,
   author = {{Hawley}, J.~F.},
    title = "{Global Magnetohydrodynamic Simulations of Cylindrical Keplerian Disks}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0011501},
 keywords = {Accretion, Accretion Disks, Black Hole Physics, Instabilities, Magnetohydrodynamics: MHD},
     year = 2001,
    month = jun,
   volume = 554,
    pages = {534-547},
      doi = {10.1086/321348},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...554..534H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001ApJ...548..348H,
   author = {{Hawley}, J.~F. and {Krolik}, J.~H.},
    title = "{Global MHD Simulation of the Inner Accretion Disk in a Pseudo-Newtonian Potential}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0006456},
 keywords = {Accretion, Accretion Disks, Instabilities, Magnetohydrodynamics: MHD, Black Hole Physics},
     year = 2001,
    month = feb,
   volume = 548,
    pages = {348-367},
      doi = {10.1086/318678},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...548..348H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001MNRAS.322..461S,
   author = {{Stone}, J.~M. and {Pringle}, J.~E.},
    title = "{Magnetohydrodynamical non-radiative accretion flows in two dimensions}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/0009233},
 keywords = {ACCRETION, ACCRETION DISCS, BLACK HOLE PHYSICS, MHD},
     year = 2001,
    month = apr,
   volume = 322,
    pages = {461-472},
      doi = {10.1046/j.1365-8711.2001.04138.x},
   adsurl = {http://adsabs.harvard.edu/abs/2001MNRAS.322..461S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1998AIPC..431...99G,
   author = {{Gammie}, C.~F.},
    title = "{Numerical models of accretion disks}",
 keywords = {Accretion and accretion disks, Infall, accretion, and accretion disks, Magnetohydrodynamics and plasmas},
booktitle = {American Institute of Physics Conference Series},
     year = 1998,
   series = {American Institute of Physics Conference Series},
   volume = 431,
   eprint = {arXiv:astro-ph/9712233},
   editor = {{Holt}, S.~S. and {Kallman}, T.~R.},
    month = apr,
    pages = {99-107},
      doi = {10.1063/1.55861},
   adsurl = {http://adsabs.harvard.edu/abs/1998AIPC..431...99G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1998tbha.conf...61B,
   author = {{Brandenburg}, A.},
    title = "{Disc turbulence and viscosity}",
booktitle = {Theory of Black Hole Accretion Disks},
     year = 1998,
   editor = {{Abramowicz}, M.~A. and {Bjornsson}, G. and {Pringle}, J.~E.
	},
    pages = {61},
   adsurl = {http://adsabs.harvard.edu/abs/1998tbha.conf...61B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007MNRAS.376.1740K,
   author = {{King}, A.~R. and {Pringle}, J.~E. and {Livio}, M.},
    title = "{Accretion disc viscosity: how big is alpha?}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/0701803},
 keywords = {accretion, accretion discs},
     year = 2007,
    month = apr,
   volume = 376,
    pages = {1740-1746},
      doi = {10.1111/j.1365-2966.2007.11556.x},
   adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.376.1740K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012MNRAS.420.2419F,
   author = {{Flaig}, M. and {Ruoff}, P. and {Kley}, W. and {Kissmann}, R.
	},
    title = "{Global structure of magnetorotationally turbulent protoplanetary discs}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1111.5497},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion discs, magnetic fields, MHD, radiative transfer, turbulence, protoplanetary discs},
     year = 2012,
    month = mar,
   volume = 420,
    pages = {2419-2428},
      doi = {10.1111/j.1365-2966.2011.20207.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.420.2419F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010MNRAS.409.1297F,
   author = {{Flaig}, M. and {Kley}, W. and {Kissmann}, R.},
    title = "{Vertical structure and turbulent saturation level in fully radiative protoplanetary disc models}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1007.4747},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion discs, instabilities, MHD, radiative transfer, turbulence, protoplanetary discs},
     year = 2010,
    month = dec,
   volume = 409,
    pages = {1297-1306},
      doi = {10.1111/j.1365-2966.2010.17392.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.409.1297F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1977A&A....55...95L,
   author = {{Livio}, M. and {Shaviv}, G.},
    title = "{On the Stability of Accretion Disks}",
  journal = {\aap},
     year = 1977,
    month = feb,
   volume = 55,
    pages = {95},
   adsurl = {http://adsabs.harvard.edu/abs/1977A%26A....55...95L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1980MNRAS.191..135T,
   author = {{Tayler}, R.~J.},
    title = "{Vertical energy transport in optically thick steady accretion discs}",
  journal = {\mnras},
 keywords = {ASTROPHYSICS, ENERGY TRANSFER, STELLAR MASS ACCRETION, CONVECTION, GAS PRESSURE, OPTICAL THICKNESS, RADIATION PRESSURE, SUPERMASSIVE STARS, VISCOSITY},
     year = 1980,
    month = apr,
   volume = 191,
    pages = {135-150},
   adsurl = {http://adsabs.harvard.edu/abs/1980MNRAS.191..135T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1987MNRAS.225..607L,
   author = {{Lin}, D.~N.~C. and {Pringle}, J.~E.},
    title = "{A viscosity prescription for a self-gravitating accretion disc}",
  journal = {\mnras},
 keywords = {ACCRETION DISKS, ANGULAR MOMENTUM, GAS VISCOSITY, GRAVITATIONAL EFFECTS, MOMENTUM TRANSFER, SIMILARITY THEOREM, STELLAR EVOLUTION},
     year = 1987,
    month = apr,
   volume = 225,
    pages = {607-613},
   adsurl = {http://adsabs.harvard.edu/abs/1987MNRAS.225..607L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009ApJ...704..281R,
   author = {{Rafikov}, R.~R.},
    title = "{Properties of Gravitoturbulent Accretion Disks}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0901.4739},
 primaryClass = "astro-ph.EP",
 keywords = {accretion, accretion disks, instabilities, planetary systems: protoplanetary disks, quasars: general},
     year = 2009,
    month = oct,
   volume = 704,
    pages = {281-291},
      doi = {10.1088/0004-637X/704/1/281},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...704..281R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1937MNRAS..97..423R,
   author = {{Robertson}, H.~P.},
    title = "{Dynamical effects of radiation in the solar system}",
  journal = {\mnras},
     year = 1937,
    month = apr,
   volume = 97,
    pages = {423},
   adsurl = {http://adsabs.harvard.edu/abs/1937MNRAS..97..423R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1962ApJ...135..855G,
   author = {{Guess}, A.~W.},
    title = "{Poynting-Robertson effect for a spherical source of radiation}",
  journal = {\apj},
     year = 1962,
    month = may,
   volume = 135,
    pages = {855-866},
      doi = {10.1086/147329},
   adsurl = {http://adsabs.harvard.edu/abs/1962ApJ...135..855G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1972AZh....49..921S,
   author = {{Shakura}, N.~I.},
    title = "{Disk Model of Gas Accretion on a Relativistic Star in a Close Binary System.}",
  journal = {\azh},
     year = 1972,
    month = oct,
   volume = 49,
    pages = {921},
   adsurl = {http://adsabs.harvard.edu/abs/1972AZh....49..921S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1977MNRAS.178..195P,
   author = {{Pringle}, J.~E.},
    title = "{Soft X-ray emission from dwarf novae}",
  journal = {\mnras},
 keywords = {BINARY STARS, COMPANION STARS, NOVAE, STELLAR LUMINOSITY, WHITE DWARF STARS, X RAY SOURCES, BLACK BODY RADIATION, BOUNDARY LAYERS, DISKS (SHAPES), MAIN
SEQUENCE STARS, STELLAR MASS, STELLAR STRUCTURE, STELLAR SYSTEMS},
     year = 1977,
    month = jan,
   volume = 178,
    pages = {195-202},
   adsurl = {http://adsabs.harvard.edu/abs/1977MNRAS.178..195P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1969Natur.223..690L,
   author = {{Lynden-Bell}, D.},
    title = "{Galactic Nuclei as Collapsed Old Quasars}",
  journal = {\nat},
     year = 1969,
    month = aug,
   volume = 223,
    pages = {690-694},
      doi = {10.1038/223690a0},
   adsurl = {http://adsabs.harvard.edu/abs/1969Natur.223..690L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1952ZNatA...7...87L,
   author = {{L{\"u}st}, R.},
    title = "{Die Entwicklung einer um einen Zentralk{\"o}rper rotierenden Gasmasse. I. L{\"o}sungen der hydrodynamischen Gleichungen mit turbulenter Reibung}",
  journal = {Zeitschrift Naturforschung Teil A},
     year = 1952,
   volume = 7,
    pages = {87},
   adsurl = {http://adsabs.harvard.edu/abs/1952ZNatA...7...87L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1974ApJ...187L...1L,
   author = {{Lightman}, A.~P. and {Eardley}, D.~M.},
    title = "{Black Holes in Binary Systems: Instability of Disk Accretion}",
  journal = {\apjl},
     year = 1974,
    month = jan,
   volume = 187,
    pages = {L1},
      doi = {10.1086/181377},
   adsurl = {http://adsabs.harvard.edu/abs/1974ApJ...187L...1L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1973A&A....29..179P,
   author = {{Pringle}, J.~E. and {Rees}, M.~J. and {Pacholczyk}, A.~G.},
    title = "{Accretion onto Massive Black Holes}",
  journal = {\aap},
     year = 1973,
    month = dec,
   volume = 29,
    pages = {179},
   adsurl = {http://adsabs.harvard.edu/abs/1973A%26A....29..179P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1976MNRAS.175..613S,
   author = {{Shakura}, N.~I. and {Sunyaev}, R.~A.},
    title = "{A theory of the instability of disk accretion on to black holes and the variability of binary X-ray sources, galactic nuclei and quasars}",
  journal = {\mnras},
 keywords = {BINARY STARS, BLACK HOLES (ASTRONOMY), GALACTIC NUCLEI, QUASARS, THERMAL INSTABILITY, X RAY SOURCES, ASYMPTOTIC METHODS, DISKS (SHAPES), PERTURBATION THEORY,
STANDING WAVES, TRAVELING WAVES},
     year = 1976,
    month = jun,
   volume = 175,
    pages = {613-632},
   adsurl = {http://adsabs.harvard.edu/abs/1976MNRAS.175..613S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1976MNRAS.177...65P,
   author = {{Pringle}, J.~E.},
    title = "{Thermal instabilities in accretion discs}",
  journal = {\mnras},
 keywords = {ASTRONOMICAL MODELS, DEPOSITION, RADIATIVE TRANSFER, THERMAL INSTABILITY, BREMSSTRAHLUNG, ELECTRON SCATTERING, PERTURBATION THEORY, RADIATION PRESSURE,
SPECTRUM ANALYSIS, X RAY STARS},
     year = 1976,
    month = oct,
   volume = 177,
    pages = {65-71},
   adsurl = {http://adsabs.harvard.edu/abs/1976MNRAS.177...65P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1975PThPh..54..706S,
   author = {{Shibazaki}, N. and {H{\= o}shi}, R.},
    title = "{Structure and Stability of Accretion-Disk around a Black-Hole}",
  journal = {Prog.~Theor.~Phys.},
     year = 1975,
    month = sep,
   volume = 54,
    pages = {706-718},
      doi = {10.1143/PTP.54.706},
   adsurl = {http://adsabs.harvard.edu/abs/1975PThPh..54..706S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1978ApJ...221..652P,
   author = {{Piran}, T.},
    title = "{The role of viscosity and cooling mechanisms in the stability of accretion disks}",
  journal = {\apj},
 keywords = {COOLING, STELLAR MASS ACCRETION, STELLAR MODELS, THERMAL STABILITY, VISCOSITY, BINARY STARS, BLACK HOLES (ASTRONOMY), DISKS (SHAPES), X RAY STARS},
     year = 1978,
    month = apr,
   volume = 221,
    pages = {652-660},
      doi = {10.1086/156069},
   adsurl = {http://adsabs.harvard.edu/abs/1978ApJ...221..652P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1998MNRAS.295L..11G,
   author = {{Godon}, P. and {Livio}, M. and {Lubow}, S.},
    title = "{Spiral shocks in accretion discs}",
  journal = {\mnras},
 keywords = {ACCRETION DISKS, COMPANION STARS, STELLAR STRUCTURE, COMPUTATIONAL ASTROPHYSICS, CATACLYSMIC VARIABLES, DWARF NOVAE, TWO DIMENSIONAL MODELS, ECLIPSING BINARY
STARS},
     year = 1998,
    month = mar,
   volume = 295,
    pages = {L11-L14},
      doi = {10.1046/j.1365-8711.1998.29510584.x},
   adsurl = {http://adsabs.harvard.edu/abs/1998MNRAS.295L..11G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1997MNRAS.292..321Y,
   author = {{Yukawa}, H. and {Boffin}, H.~M.~J. and {Matsuda}, T.},
    title = "{Spiral shocks in three-dimensional accretion discs}",
  journal = {\mnras},
 keywords = {ACCRETION DISKS, THREE DIMENSIONAL MODELS, HYDRODYNAMIC EQUATIONS, SHOCK WAVE PROFILES, BINARY STARS, HYDROSTATIC PRESSURE, DIGITAL SIMULATION, HIGH
TEMPERATURE GASES},
     year = 1997,
    month = dec,
   volume = 292,
    pages = {321},
   adsurl = {http://adsabs.harvard.edu/abs/1997MNRAS.292..321Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1979MNRAS.187..777P,
   author = {{Pringle}, J.~E. and {Savonije}, G.~J.},
    title = "{X-ray emission from dwarf novae}",
  journal = {\mnras},
 keywords = {NOVAE, STELLAR RADIATION, WHITE DWARF STARS, X RAY SOURCES, BOUNDARY LAYERS, DEPOSITION, HIGH TEMPERATURE, OPTICAL THICKNESS},
     year = 1979,
    month = jun,
   volume = 187,
    pages = {777-783},
   adsurl = {http://adsabs.harvard.edu/abs/1979MNRAS.187..777P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1981AcA....31..267T,
   author = {{Tylenda}, R.},
    title = "{Viscous Boundary Layer and Hard X-Rays from Dwarf Novae}",
  journal = {\actaa},
     year = 1981,
   volume = 31,
    pages = {267},
   adsurl = {http://adsabs.harvard.edu/abs/1981AcA....31..267T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1983A&A...126..146R,
   author = {{Regev}, O.},
    title = "{The disk-star boundary layer and its effect on the accretion disk structure}",
  journal = {\aap},
 keywords = {ACCRETION DISKS, BINARY STARS, STELLAR MASS ACCRETION, VARIABLE STARS, WHITE DWARF STARS, ASYMPTOTIC METHODS, MATHEMATICAL MODELS, STELLAR MODELS, X RAYS},
     year = 1983,
    month = sep,
   volume = 126,
    pages = {146-151},
   adsurl = {http://adsabs.harvard.edu/abs/1983A%26A...126..146R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1991A&A...247...95K,
   author = {{Kley}, W.},
    title = "{On the influence of the viscosity on the structure of the boundary layer of accretion disks}",
  journal = {\aap},
 keywords = {ACCRETION DISKS, CATACLYSMIC VARIABLES, STELLAR STRUCTURE, BOUNDARY LAYERS, COMPUTATIONAL ASTROPHYSICS, HYDRODYNAMICS, PROTOSTARS, VISCOSITY},
     year = 1991,
    month = jul,
   volume = 247,
    pages = {95-107},
   adsurl = {http://adsabs.harvard.edu/abs/1991A%26A...247...95K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@PHDTHESIS{1987PhDT.......161K,
   author = {{Klu{\'z}niak}, W.},
   school = {, Stanford Univ., (1987)},
     year = 1987,
   adsurl = {http://adsabs.harvard.edu/abs/1987PhDT.......161K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1988ApJ...333..227C,
   author = {{Cannizzo}, J.~K. and {Shafter}, A.~W. and {Wheeler}, J.~C.},
    title = "{On the outburst recurrence time for the accretion disk limit cycle mechanism in dwarf novae}",
  journal = {\apj},
 keywords = {ACCRETION DISKS, CATACLYSMIC VARIABLES, DWARF NOVAE, STELLAR PHYSICS, LATE STARS, MASS TRANSFER, STELLAR MASS ACCRETION, STELLAR ORBITS, WHITE DWARF STARS},
     year = 1988,
    month = oct,
   volume = 333,
    pages = {227-235},
      doi = {10.1086/166739},
   adsurl = {http://adsabs.harvard.edu/abs/1988ApJ...333..227C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1980MNRAS.190...87C,
   author = {{Cordova}, F.~A. and {Nugent}, J.~J. and {Klein}, S.~R. and 
	{Garmire}, G.~P.},
    title = "{The HEAO-A2 soft X-ray survey of dwarf novae in outburst}",
  journal = {\mnras},
 keywords = {DWARF STARS, NOVAE, SPACEBORNE ASTRONOMY, STELLAR RADIATION, X RAY ASTRONOMY, BRIGHTNESS TEMPERATURE, BURSTS, GAS DENSITY, HEAO 1, HYDROGEN, LIGHT CURVE,
ULTRAVIOLET SPECTRA, X RAY SPECTRA},
     year = 1980,
    month = jan,
   volume = 190,
    pages = {87-97},
   adsurl = {http://adsabs.harvard.edu/abs/1980MNRAS.190...87C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2004RMxAC..20..174M,
   author = {{Mauche}, C.~W.},
    title = "{A Simple, Unifying Model of the Extreme Ultraviolet Spectra of Dwarf Novae in Outburst}",
 keywords = {Binaries: Close, Novae, Cataclysmic variables, Stars: Individual (SS Cyg, WZ Sge), Stars: Winds, outflows, Ultraviolet: Stars},
booktitle = {Revista Mexicana de Astronomia y Astrofisica Conference Series},
     year = 2004,
   series = {Revista Mexicana de Astronomia y Astrofisica Conference Series},
   volume = 20,
   editor = {{Tovmassian}, G. and {Sion}, E.},
    month = jul,
    pages = {174-175},
   adsurl = {http://adsabs.harvard.edu/abs/2004RMxAC..20..174M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1999MNRAS.303..603O,
   author = {{Obach}, C. and {Glatzel}, W.},
    title = "{On the boundary layer of accretion discs}",
  journal = {\mnras},
 keywords = {ACCRETION, ACCRETION DISCS, HYDRODYNAMICS, NOVAE, CATACLYSMIC VARIABLES},
     year = 1999,
    month = mar,
   volume = 303,
    pages = {603-610},
      doi = {10.1046/j.1365-8711.1999.02278.x},
   adsurl = {http://adsabs.harvard.edu/abs/1999MNRAS.303..603O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2004RMxAC..20..244M,
   author = {{Mukai}, K. and {Patterson}, J.},
    title = "{XMM-Newton and Optical Observations of WZ Sagittae in Quiescence}",
booktitle = {Revista Mexicana de Astronomia y Astrofisica Conference Series},
     year = 2004,
   series = {Revista Mexicana de Astronomia y Astrofisica Conference Series},
   volume = 20,
   editor = {{Tovmassian}, G. and {Sion}, E.},
    month = jul,
    pages = {244-244},
   adsurl = {http://adsabs.harvard.edu/abs/2004RMxAC..20..244M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003MNRAS.346.1231P,
   author = {{Pandel}, D. and {C{\'o}rdova}, F.~A. and {Howell}, S.~B.},
    title = "{X-ray and ultraviolet observations of the dwarf nova VW Hyi in quiescence}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/0309418},
 keywords = {accretion, accretion discs, binaries: close, stars: dwarf novae, stars: individual: VW Hyi, novae, cataclysmic variables, X-rays: stars},
     year = 2003,
    month = dec,
   volume = 346,
    pages = {1231-1241},
      doi = {10.1111/j.1365-2966.2003.07199.x},
   adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.346.1231P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005ApJ...626..396P,
   author = {{Pandel}, D. and {C{\'o}rdova}, F.~A. and {Mason}, K.~O. and 
	{Priedhorsky}, W.~C.},
    title = "{X-Ray Observations of the Boundary Layer in Dwarf Novae at Low Accretion Rates}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0503114},
 keywords = {Accretion, Accretion Disks, Stars: Binaries: Close, Stars: Novae, Cataclysmic Variables, Stars: Dwarf Novae, Stars: Individual: Constellation Name: OY
Carinae, Stars: Individual: Constellation Name: WW Ceti, Stars: Individual: Constellation Name: AB Draconis, Stars: Individual: Constellation Name: U Geminorum, Stars:
Individual: Constellation Name: VW Hydri, Stars: Individual: Constellation Name: WX Hydri, Stars: Individual: Constellation Name: T Leonis, Stars: Individual:
Constellation Name: TY Piscis Austrini, Stars: Individual: Constellation Name: EI Ursae Majoris, Stars: Individual: Constellation Name: SU Ursae Majoris, X-Rays:
Binaries},
     year = 2005,
    month = jun,
   volume = 626,
    pages = {396-410},
      doi = {10.1086/429983},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...626..396P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1984Natur.308..519K,
   author = {{King}, A.~R. and {Shaviv}, G.},
    title = "{X-ray emission from non-magnetic cataclysmic variables}",
  journal = {\nat},
 keywords = {BINARY STARS, STELLAR RADIATION, VARIABLE STARS, WHITE DWARF STARS, X RAY SOURCES, BOUNDARY LAYER FLOW, STELLAR CORONAS, STELLAR MASS ACCRETION},
     year = 1984,
    month = apr,
   volume = 308,
    pages = {519-521},
      doi = {10.1038/308519a0},
   adsurl = {http://adsabs.harvard.edu/abs/1984Natur.308..519K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1987Ap&SS.130..303S,
   author = {{Shaviv}, G.},
    title = "{The boundary layer in cataclysmic variables}",
  journal = {\apss},
 keywords = {ACCRETION DISKS, BOUNDARY LAYERS, CATACLYSMIC VARIABLES, WHITE DWARF STARS, MIXING, STELLAR CORONAS, STELLAR INTERIORS},
     year = 1987,
    month = feb,
   volume = 130,
    pages = {303-314},
      doi = {10.1007/BF00655010},
   adsurl = {http://adsabs.harvard.edu/abs/1987Ap%26SS.130..303S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1993Natur.362..820N,
   author = {{Narayan}, R. and {Popham}, R.},
    title = "{Hard X-rays from accretion disk boundary layers}",
  journal = {\nat},
 keywords = {ACCRETION DISKS, BOUNDARY LAYER FLOW, LUMINOSITY, WHITE DWARF STARS, X RAY SPECTRA, CATACLYSMIC VARIABLES, SELF CONSISTENT FIELDS, STELLAR MASS ACCRETION,
TEMPERATURE DISTRIBUTION},
     year = 1993,
    month = apr,
   volume = 362,
    pages = {820-822},
      doi = {10.1038/362820a0},
   adsurl = {http://adsabs.harvard.edu/abs/1993Natur.362..820N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1999MNRAS.308..979P,
   author = {{Popham}, R.},
    title = "{A boundary layer origin for dwarf nova oscillations}",
  journal = {\mnras},
     year = 1999,
    month = oct,
   volume = 308,
    pages = {979-983},
      doi = {10.1046/j.1365-8711.1999.02782.x},
   adsurl = {http://adsabs.harvard.edu/abs/1999MNRAS.308..979P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1995A&A...300..823L,
   author = {{Liu}, F.~K. and {Meyer}, F. and {Meyer-Hofmeister}, E.},
    title = "{Dwarf novae in quiescence: the relationship between disk evaporation and accretion onto a white dwarf.}",
  journal = {\aap},
 keywords = {ACCRETION, ACCRETION DISK, CATACLYSMIC VARIABLES, STARS: CORONAE, WHITE DWARFS, X-RAYS:STARS, ULTRAVIOLET: STARS},
     year = 1995,
    month = aug,
   volume = 300,
    pages = {823},
   adsurl = {http://adsabs.harvard.edu/abs/1995A%26A...300..823L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001ApJ...554.1255M,
   author = {{Medvedev}, M.~V. and {Narayan}, R.},
    title = "{Self-similar Hot Accretion Flow onto a Neutron Star}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0007064},
 keywords = {Accretion, Accretion Disks, Stars: Neutron},
     year = 2001,
    month = jun,
   volume = 554,
    pages = {1255-1267},
      doi = {10.1086/321385},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...554.1255M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1994A&A...288..175M,
   author = {{Meyer}, F. and {Meyer-Hofmeister}, E.},
    title = "{Accretion disk evaporation by a coronal siphon flow}",
  journal = {\aap},
 keywords = {ACCRETION DISKS, DWARF NOVAE, MASS FLOW, STELLAR CORONAS, ULTRAVIOLET EMISSION, WHITE DWARF STARS, X RAYS, BOUNDARY CONDITIONS, MASS FLOW RATE, MATHEMATICAL
MODELS, STELLAR MODELS, STELLAR WINDS, TEMPERATURE DISTRIBUTION, X RAY SPECTRA},
     year = 1994,
    month = aug,
   volume = 288,
    pages = {175-182},
   adsurl = {http://adsabs.harvard.edu/abs/1994A%26A...288..175M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008A&A...483..231L,
   author = {{Liu}, F.~K. and {Meyer}, F. and {Meyer-Hofmeister}, E. and 
	{Burwitz}, V.},
    title = "{Low heat conduction in white dwarf boundary layers?}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0803.1894},
 keywords = {stars: dwarf novae, accretion, accretion disks, X-rays: individuals: VW Hyi, conduction, magnetic fields, galaxies: cooling flows},
     year = 2008,
    month = may,
   volume = 483,
    pages = {231-237},
      doi = {10.1051/0004-6361:20079260},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...483..231L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1991MNRAS.249..452H,
   author = {{Hoare}, M.~G. and {Drew}, J.~E.},
    title = "{Boundary-layer temperatures in high accretion rate cataclysmic variables}",
  journal = {\mnras},
 keywords = {ACCRETION DISKS, CATACLYSMIC VARIABLES, DWARF NOVAE, RADIATIVE RECOMBINATION, STELLAR ENVELOPES, BOUNDARY LAYERS, STELLAR WINDS, TEMPERATURE DISTRIBUTION,
WHITE DWARF STARS, X RAY SPECTRA},
     year = 1991,
    month = apr,
   volume = 249,
    pages = {452-459},
   adsurl = {http://adsabs.harvard.edu/abs/1991MNRAS.249..452H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1994A&A...292..519V,
   author = {{van Teeseling}, A. and {Verbunt}, F.},
    title = "{ROSAT X-ray observations of ten cataclysmic variables}",
  journal = {\aap},
 keywords = {ACCRETION DISKS, CATACLYSMIC VARIABLES, STELLAR MASS ACCRETION, ULTRAVIOLET ASTRONOMY, ULTRAVIOLET SPECTRA, VARIABILITY, X RAY ASTRONOMY, X RAY SPECTRA, X
RAY STARS, EXOSAT SATELLITE, HEAO 2, HYDROGEN, IMAGE PROCESSING, LIGHT CURVE, PROPORTIONAL COUNTERS, ROSAT MISSION, STATISTICAL ANALYSIS, X RAY TELESCOPES},
     year = 1994,
    month = dec,
   volume = 292,
    pages = {519-533},
   adsurl = {http://adsabs.harvard.edu/abs/1994A%26A...292..519V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1982ApJ...262L..53F,
   author = {{Ferland}, G.~J. and {Pepper}, G.~H. and {Langer}, S.~H. and 
	{MacDonald}, J. and {Truran}, J.~W. and {Shaviv}, G.},
    title = "{The mystery of the missing boundary layer}",
  journal = {\apjl},
 keywords = {BINARY STARS, NOVAE, STELLAR MASS ACCRETION, ULTRAVIOLET ASTRONOMY, X RAY SOURCES, ACCRETION DISKS, BOUNDARY LAYERS, FAR ULTRAVIOLET RADIATION, STELLAR
MODELS},
     year = 1982,
    month = nov,
   volume = 262,
    pages = {L53-L58},
      doi = {10.1086/183910},
   adsurl = {http://adsabs.harvard.edu/abs/1982ApJ...262L..53F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1997MNRAS.288L..16K,
   author = {{King}, A.~R.},
    title = "{The UV delay in dwarf novae}",
  journal = {\mnras},
 keywords = {ACCRETION, ACCRETION DISCS, INSTABILITIES, NOVAE, CATACLYSMIC VARIABLES, ULTRAVIOLET: STARS},
     year = 1997,
    month = jun,
   volume = 288,
    pages = {L16-L18},
   adsurl = {http://adsabs.harvard.edu/abs/1997MNRAS.288L..16K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1995MNRAS.276..495P,
   author = {{Ponman}, T.~J. and {Belloni}, T. and {Duck}, S.~R. and {Verbunt}, F. and 
	{Watson}, M.~G. and {Wheatley}, P.~J. and {Pfeffermann}, E.},
    title = "{The EUV/X-ray spectrum of SS Cygni in outburst}",
  journal = {\mnras},
 keywords = {ACCRETION, ACCRETION DISCS, BINARIES: CLOSE, STARS: INDIVIDUAL: SS CYG, NOVAE, CATACLYSMIC VARIABLES, X-RAYS: STARS},
     year = 1995,
    month = sep,
   volume = 276,
    pages = {495-504},
   adsurl = {http://adsabs.harvard.edu/abs/1995MNRAS.276..495P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1978A&A....63..265K,
   author = {{Kippenhahn}, R. and {Thomas}, H.-C.},
    title = "{Accretion belts on white dwarfs}",
  journal = {\aap},
 keywords = {NOVAE, STELLAR MASS ACCRETION, STELLAR MODELS, WHITE DWARF STARS, ASTRONOMICAL MODELS, STELLAR LUMINOSITY, STELLAR ROTATION},
     year = 1978,
    month = feb,
   volume = 63,
    pages = {265-272},
   adsurl = {http://adsabs.harvard.edu/abs/1978A%26A....63..265K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1989ApJ...340.1006R,
   author = {{Regev}, O. and {Shara}, M.~M.},
    title = "{How much boundary layer heating occurs in an accreting prenova white dwarf?}",
  journal = {\apj},
 keywords = {ACCRETION DISKS, COMPUTATIONAL ASTROPHYSICS, ENERGY TRANSFER, NOVAE, STELLAR ENVELOPES, STELLAR MASS ACCRETION, WHITE DWARF STARS, ASYMPTOTIC METHODS,
BOUNDARY LAYERS, HEATING, OPTICAL THICKNESS, STELLAR ATMOSPHERES, STELLAR ROTATION},
     year = 1989,
    month = may,
   volume = 340,
    pages = {1006-1010},
      doi = {10.1086/167453},
   adsurl = {http://adsabs.harvard.edu/abs/1989ApJ...340.1006R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1997ApJ...478..734P,
   author = {{Popham}, R.},
    title = "{Heating of a Star by Disk Accretion}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/9610131},
 keywords = {ACCRETION, ACCRETION DISKS, RADIATIVE TRANSFER, STARS: NOVAE, CATACLYSMIC VARIABLES, STARS: PRE-MAIN-SEQUENCE},
     year = 1997,
    month = mar,
   volume = 478,
    pages = {734},
      doi = {10.1086/303806},
   adsurl = {http://adsabs.harvard.edu/abs/1997ApJ...478..734P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1997ApJ...484L.149C,
   author = {{Cheng}, F.~H. and {Sion}, E.~M. and {Szkody}, P. and {Huang}, M.
	},
    title = "{Hubble Space Telescope Observations of the Dwarf Nova WZ Sagittae: A Very Rapidly Rotating White Dwarf}",
  journal = {\apjl},
 keywords = {STARS: NOVAE, CATACLYSMIC VARIABLES, STARS: INDIVIDUAL CONSTELLATION NAME: WZ SAGITTAE, STARS: WHITE DWARFS},
     year = 1997,
    month = aug,
   volume = 484,
    pages = {L149},
      doi = {10.1086/310794},
   adsurl = {http://adsabs.harvard.edu/abs/1997ApJ...484L.149C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005MNRAS.361..809G,
   author = {{Godon}, P. and {Sion}, E.~M.},
    title = "{The boundary layer of VW Hydri in quiescence}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/0406370},
 keywords = {accretion, accretion discs, stars: individual: VW Hyi, novae, cataclysmic variables},
     year = 2005,
    month = aug,
   volume = 361,
    pages = {809-812},
      doi = {10.1111/j.1365-2966.2005.09209.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.361..809G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010AstL...36..848I,
   author = {{Inogamov}, N.~A. and {Sunyaev}, R.~A.},
    title = "{Spread of matter over a neutron-star surface during disk accretion: Deceleration of rapid rotation}",
  journal = {Astron.~Lett.},
archivePrefix = "arXiv",
   eprint = {1102.0975},
 primaryClass = "astro-ph.HE",
 keywords = {disk accretion, neutron stars, boundary layer, X-ray sources, X-ray bursters, low-mass X-ray binaries},
     year = 2010,
    month = dec,
   volume = 36,
    pages = {848-894},
      doi = {10.1134/S1063773710120029},
   adsurl = {http://adsabs.harvard.edu/abs/2010AstL...36..848I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001ApJ...547..355P,
   author = {{Popham}, R. and {Sunyaev}, R.},
    title = "{Accretion Disk Boundary Layers around Neutron Stars: X-Ray Production in Low-Mass X-Ray Binaries}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0004017},
 keywords = {Accretion, Accretion Disks, Stars: Binaries: Close, Stars: Neutron, X-Rays: Stars},
     year = 2001,
    month = jan,
   volume = 547,
    pages = {355-383},
      doi = {10.1086/318336},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...547..355P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004ApJ...610..977P,
   author = {{Piro}, A.~L. and {Bildsten}, L.},
    title = "{Spreading of Accreted Material on White Dwarfs}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0404214},
 keywords = {Accretion, Accretion Disks, Stars: Novae, Cataclysmic Variables, Stars: Dwarf Novae, Stars: White Dwarfs, X-Rays: Stars},
     year = 2004,
    month = aug,
   volume = 610,
    pages = {977-990},
      doi = {10.1086/421763},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...610..977P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004ApJ...616L.155P,
   author = {{Piro}, A.~L. and {Bildsten}, L.},
    title = "{A Spreading Layer Origin for Dwarf Nova Oscillations}",
  journal = {\apjl},
   eprint = {arXiv:astro-ph/0410427},
 keywords = {Accretion, Accretion Disks, Stars: Novae, Cataclysmic Variables, Stars: Individual: Constellation Name: SS Cygni, Stars: Oscillations, Stars: White Dwarfs},
     year = 2004,
    month = dec,
   volume = 616,
    pages = {L155-L158},
      doi = {10.1086/426501},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...616L.155P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006MNRAS.369.2036S,
   author = {{Suleimanov}, V. and {Poutanen}, J.},
    title = "{Spectra of the spreading layers on the neutron star surface and constraints on the neutron star equation of state}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/0601689},
 keywords = {accretion, accretion discs: radiative transfer: stars: neutron: X-rays: binaries, accretion discs, radiative transfer, stars: neutron, X-rays: binaries},
     year = 2006,
    month = jul,
   volume = 369,
    pages = {2036-2048},
      doi = {10.1111/j.1365-2966.2006.10454.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.369.2036S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1998ApJ...502..730C,
   author = {{Collins}, T.~J.~B. and {Helfer}, H.~L. and {van Horn}, H.~M.
	},
    title = "{Accretion Disk and Boundary Layer Models Incorporating OPAL Opacities}",
  journal = {\apj},
 keywords = {ACCRETION, ACCRETION DISKS, STARS: NOVAE, CATACLYSMIC VARIABLES},
     year = 1998,
    month = aug,
   volume = 502,
    pages = {730},
      doi = {10.1086/305949},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...502..730C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1981ApJ...248..321L,
   author = {{Levermore}, C.~D. and {Pomraning}, G.~C.},
    title = "{A flux-limited diffusion theory}",
  journal = {\apj},
 keywords = {DIFFUSION THEORY, RADIANT FLUX DENSITY, RADIATIVE TRANSFER, TRANSPORT THEORY, BOLTZMANN TRANSPORT EQUATION, BOUNDARY VALUE PROBLEMS, DIFFUSION COEFFICIENT,
GASEOUS DIFFUSION},
     year = 1981,
    month = aug,
   volume = 248,
    pages = {321-334},
      doi = {10.1086/159157},
   adsurl = {http://adsabs.harvard.edu/abs/1981ApJ...248..321L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1984JQSRT..31..149L,
   author = {{Levermore}, C.~D.},
    title = "{Relating Eddington factors to flux limiters.}",
  journal = {\jqsrt},
 keywords = {Radiative Transfer},
     year = 1984,
    month = feb,
   volume = 31,
    pages = {149-160},
      doi = {10.1016/0022-4073(84)90112-2},
   adsurl = {http://adsabs.harvard.edu/abs/1984JQSRT..31..149L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1999ApJ...518..833K,
   author = {{Kley}, W. and {Lin}, D.~N.~C.},
    title = "{Evolution of FU Orionis Outbursts in Protostellar Disks}",
  journal = {\apj},
 keywords = {ACCRETION, ACCRETION DISKS, STARS: CIRCUMSTELLAR MATTER, HYDRODYNAMICS, STARS: FORMATION, STARS: PRE-MAIN-SEQUENCE, STARS: VARIABLES: OTHER (FU ORIONIS)},
     year = 1999,
    month = jun,
   volume = 518,
    pages = {833-847},
      doi = {10.1086/307296},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...518..833K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005ApJ...635L..69F,
   author = {{Fisker}, J.~L. and {Balsara}, D.~S.},
    title = "{Simulating the Boundary Layer between a White Dwarf and Its Accretion Disk}",
  journal = {\apjl},
 keywords = {Accretion, Accretion Disks, Stars: Binaries: Close, Methods: Numerical, Stars: Novae, Cataclysmic Variables, Stars: White Dwarfs},
     year = 2005,
    month = dec,
   volume = 635,
    pages = {L69-L72},
      doi = {10.1086/499159},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...635L..69F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2006NewAR..50..509F,
   author = {{Fisker}, J.~L. and {Balsara}, D.~S. and {Burger}, T.},
    title = "{The accretion and spreading of matter on white dwarfs}",
  journal = {\nar},
     year = 2006,
    month = oct,
   volume = 50,
    pages = {509-515},
      doi = {10.1016/j.newar.2006.06.009},
   adsurl = {http://adsabs.harvard.edu/abs/2006NewAR..50..509F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003ApJ...589..397K,
   author = {{K{\"u}ker}, M. and {Henning}, T. and {R{\"u}diger}, G.},
    title = "{Magnetic Star-Disk Coupling in Classical T Tauri Systems}",
  journal = {\apj},
 keywords = {Accretion, Accretion Disks, Stars: Circumstellar Matter, Magnetohydrodynamics: MHD, Stars: Magnetic Fields, Stars: Pre-Main-Sequence, Stars: Variables:
Other},
     year = 2003,
    month = may,
   volume = 589,
    pages = {397-409},
      doi = {10.1086/374408},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...589..397K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002MNRAS.330..895A,
   author = {{Armitage}, P.~J.},
    title = "{Magnetic activity in accretion disc boundary layers}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/0110670},
 keywords = {ACCRETION, ACCRETION DISCS, MAGNETIC FIELDS, MHD, NOVAE, CATACLYSMIC VARIABLES, STARS: PRE-MAIN-SEQUENCE, STARS: WINDS, OUTFLOWS, accretion, accretion discs;
magnetic fields; MHD; novae, cataclysmic variables; stars: pre-main-sequence; stars: winds, outflows},
     year = 2002,
    month = mar,
   volume = 330,
    pages = {895-900},
      doi = {10.1046/j.1365-8711.2002.05152.x},
   adsurl = {http://adsabs.harvard.edu/abs/2002MNRAS.330..895A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008MNRAS.386.1038B,
   author = {{Babkovskaia}, N. and {Brandenburg}, A. and {Poutanen}, J.},
    title = "{Boundary layer on the surface of a neutron star}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0802.1663},
 keywords = {accretion, accretion discs , hydrodynamics , stars: neutron},
     year = 2008,
    month = may,
   volume = 386,
    pages = {1038-1044},
      doi = {10.1111/j.1365-2966.2008.13099.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.386.1038B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012MNRAS.421...63R,
   author = {{Romanova}, M.~M. and {Ustyugova}, G.~V. and {Koldoba}, A.~V. and 
	{Lovelace}, R.~V.~E.},
    title = "{MRI-driven accretion on to magnetized stars: global 3D MHD simulations of magnetospheric and boundary layer regimes}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1111.3068},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion discs, instabilities, magnetic fields, plasmas},
     year = 2012,
    month = mar,
   volume = 421,
    pages = {63-77},
      doi = {10.1111/j.1365-2966.2011.20055.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.421...63R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1978MNRAS.185..629K,
   author = {{Kato}, S.},
    title = "{Pulsational instability of accretion disks to axially symmetric oscillations}",
  journal = {\mnras},
     year = 1978,
    month = dec,
   volume = 185,
    pages = {629-642},
   adsurl = {http://adsabs.harvard.edu/abs/1978MNRAS.185..629K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1984ApJ...287..774B,
   author = {{Blumenthal}, G.~R. and {Lin}, D.~N.~C. and {Yang}, L.~T.},
    title = "{On the overstability of axisymmetric oscillations in thin accretion disks}",
  journal = {\apj},
 keywords = {ACCRETION DISKS, DWARF NOVAE, MOTION STABILITY, OPTICAL THICKNESS, STELLAR MASS ACCRETION, STELLAR OSCILLATIONS, AXISYMMETRIC BODIES, DIFFERENTIAL EQUATIONS,
ELECTRON SCATTERING, HIGH REYNOLDS NUMBER, LAMINAR FLOW, PERTURBATION THEORY, STEADY STATE},
     year = 1984,
    month = dec,
   volume = 287,
    pages = {774-784},
      doi = {10.1086/162736},
   adsurl = {http://adsabs.harvard.edu/abs/1984ApJ...287..774B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1986MNRAS.220..593P,
   author = {{Papaloizou}, J.~C.~B. and {Stanley}, G.~Q.~G.},
    title = "{The structure and stability of the accretion disc boundary layer}",
  journal = {\mnras},
 keywords = {ACCRETION DISKS, BOUNDARY LAYER STABILITY, MAGNETOHYDRODYNAMIC STABILITY, STELLAR MODELS, STELLAR STRUCTURE, PERTURBATION THEORY, STEADY STATE, STELLAR
OSCILLATIONS, VISCOSITY},
     year = 1986,
    month = jun,
   volume = 220,
    pages = {593-610},
   adsurl = {http://adsabs.harvard.edu/abs/1986MNRAS.220..593P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1994MNRAS.268...29P,
   author = {{Papaloizou}, J. and {Szuszkiewicz}, E.},
    title = "{A Comparison of One-Dimensional and Two-Dimensional Models of Transonic Accretion Discs around Collapsed Objects}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/9401025},
 keywords = {accretion, accretion discs - hydrodynamics - celestial mechanics, stellar dynamics},
     year = 1994,
    month = may,
   volume = 268,
    pages = {29},
   adsurl = {http://adsabs.harvard.edu/abs/1994MNRAS.268...29P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1994ApJ...431..359N,
   author = {{Narayan}, R. and {Loeb}, A. and {Kumar}, P.},
    title = "{Casuality in strong shear flows}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/9401004},
 keywords = {ACCRETION DISKS, FLOW DISTRIBUTION, PARTICLE COLLISIONS, PARTICLE DIFFUSION, SHEAR FLOW, VISCOUS FLOW, BOLTZMANN TRANSPORT EQUATION, CAUSES, COMPUTATIONAL
ASTROPHYSICS, HYDRODYNAMIC EQUATIONS, SHEAR STRESS},
     year = 1994,
    month = aug,
   volume = 431,
    pages = {359-279},
      doi = {10.1086/174490},
   adsurl = {http://adsabs.harvard.edu/abs/1994ApJ...431..359N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1994PASJ...46..289K,
   author = {{Kato}, S. and {Inagaki}, S.},
    title = "{A non-local description of turbulent stress tensor in accretion disks}",
  journal = {\pasj},
 keywords = {ACCRETION DISKS, BOUNDARY LAYERS, STELLAR ROTATION, TURBULENT FLOW, VISCOSITY, MATHEMATICAL MODELS, RADIAL FLOW, STRESS TENSORS},
     year = 1994,
    month = jun,
   volume = 46,
    pages = {289-299},
   adsurl = {http://adsabs.harvard.edu/abs/1994PASJ...46..289K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1995MNRAS.277..157G,
   author = {{Godon}, P.},
    title = "{On the turbulent viscosity prescription in accretion discs}",
  journal = {\mnras},
 keywords = {ACCRETION, ACCRETION DISCS, HYDRODYNAMICS, TURBULENCE},
     year = 1995,
    month = nov,
   volume = 277,
    pages = {157-162},
   adsurl = {http://adsabs.harvard.edu/abs/1995MNRAS.277..157G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1992ApJ...400..610B,
   author = {{Balbus}, S.~A. and {Hawley}, J.~F.},
    title = "{A Powerful Local Shear Instability in Weakly Magnetized Disks. IV. Nonaxisymmetric Perturbations}",
  journal = {\apj},
 keywords = {ACCRETION, ACCRETION DISKS, INSTABILITIES, MAGNETOHYDRODYNAMICS: MHD},
     year = 1992,
    month = dec,
   volume = 400,
    pages = {610-621},
      doi = {10.1086/172022},
   adsurl = {http://adsabs.harvard.edu/abs/1992ApJ...400..610B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1996MNRAS.281L..21A,
   author = {{Abramowicz}, M. and {Brandenburg}, A. and {Lasota}, J.-P.},
    title = "{The dependence of the viscosity in accretion discs on the shear/vorticity ratio}",
  journal = {\mnras},
 keywords = {accretion, accretion discs -- black hole physics -- turbulence},
     year = 1996,
    month = jul,
   volume = 281,
    pages = {L21},
   adsurl = {http://adsabs.harvard.edu/abs/1996MNRAS.281L..21A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1988AdSpR...8..135S,
   author = {{Shakura}, N.~I. and {Sunyaev}, R.~A.},
    title = "{The theory of an accretion disk/neutron star boundary layer}",
  journal = {Adv.~Space~Res.},
 keywords = {ACCRETION DISKS, NEUTRON STARS, PLANETARY ATMOSPHERES, STELLAR MOTIONS, ANGULAR VELOCITY, ATMOSPHERIC DENSITY, CIRCULAR ORBITS, PARTICLE ACCELERATION},
     year = 1988,
   volume = 8,
    pages = {135-140},
      doi = {10.1016/0273-1177(88)90396-1},
   adsurl = {http://adsabs.harvard.edu/abs/1988AdSpR...8..135S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1992ApJ...394..261N,
   author = {{Narayan}, R.},
    title = "{A flux-limited model of particle diffusion and viscosity}",
  journal = {\apj},
 keywords = {DIFFUSION THEORY, MATHEMATICAL MODELS, PARTICLE DIFFUSION, RADIATIVE TRANSFER, VISCOSITY, ACCRETION DISKS, BOLTZMANN TRANSPORT EQUATION, TRANSPORT THEORY,
VELOCITY DISTRIBUTION},
     year = 1992,
    month = jul,
   volume = 394,
    pages = {261-267},
      doi = {10.1086/171578},
   adsurl = {http://adsabs.harvard.edu/abs/1992ApJ...394..261N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1992ApJ...394..255P,
   author = {{Popham}, R. and {Narayan}, R.},
    title = "{Supersonic infall and causality in accretion disk boundary layers}",
  journal = {\apj},
 keywords = {ACCRETION DISKS, BOUNDARY LAYERS, STELLAR MASS ACCRETION, SUPERSONIC FLOW, COMPUTATIONAL ASTROPHYSICS, HYDRODYNAMIC EQUATIONS, RADIAL FLOW, VISCOSITY},
     year = 1992,
    month = jul,
   volume = 394,
    pages = {255-260},
      doi = {10.1086/171577},
   adsurl = {http://adsabs.harvard.edu/abs/1992ApJ...394..255P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{jou2001extended,
  title={Extended Irreversible Thermodynamics},
  author={Jou, D. and Casas-V{\'a}zquez, J. and Lebon, G.},
  isbn={9783540411567},
  lccn={00053784},
  series={Physics and Astronomy Online Library},
  url={http://books.google.de/books?id=QSGOsmZ5srUC},
  year={2001},
  publisher={Springer}
}

@ARTICLE{1972MNRAS.159..101W,
   author = {{Warner}, B. and {Robinson}, E.~L.},
    title = "{Observations of rapid variables - IX. AM CVn (HZ 29).}",
  journal = {\mnras},
     year = 1972,
   volume = 159,
    pages = {101-111},
   adsurl = {http://adsabs.harvard.edu/abs/1972MNRAS.159..101W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1977ApJ...214..144P,
   author = {{Patterson}, J. and {Robinson}, E.~L. and {Nather}, R.~E.},
    title = "{Rapid and ultrarapid oscillations in RU Pegasi.}",
  journal = {\apj},
     year = 1977,
    month = may,
   volume = 214,
    pages = {144-151},
      doi = {10.1086/155239},
   adsurl = {http://adsabs.harvard.edu/abs/1977ApJ...214..144P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008MNRAS.383.1469W,
   author = {{Warner}, B. and {Pretorius}, M.~L.},
    title = "{Dwarf nova oscillations and quasi-periodic oscillations in cataclysmic variables - VI. Spin rates, propellering and coherence}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0710.5057},
 keywords = {accretion, accretion discs , stars: dwarf novae , stars: individual: TY PsA , stars: individual: WZ Sge , stars: magnetic fields , stars: oscillations},
     year = 2008,
    month = feb,
   volume = 383,
    pages = {1469-1476},
      doi = {10.1111/j.1365-2966.2007.12645.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.383.1469W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1996ApJ...463L..87M,
   author = {{Mauche}, C.~W.},
    title = "{Quasi-coherent Oscillations in the Extreme Ultraviolet Flux of the Dwarf Nova SS Cygni}",
  journal = {\apjl},
   eprint = {arXiv:astro-ph/9603098},
 keywords = {STARS: INDIVIDUAL CONSTELLATION NAME: SS CYGNI, STARS: MAGNETIC FIELDS, STARS: NOVAE, CATACLYSMIC VARIABLES, STARS: OSCILLATIONS},
     year = 1996,
    month = jun,
   volume = 463,
    pages = {L87},
      doi = {10.1086/310070},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...463L..87M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2001ApJ...562..508M,
   author = {{Mauche}, C.~W. and {Robinson}, E.~L.},
    title = "{First Simultaneous Optical and Extreme-Ultraviolet Observations of the Quasi-coherent Oscillations of SS Cygni}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0108059},
 keywords = {Stars: Novae, Cataclysmic Variables, stars: individual (SS Cygni), Stars: Oscillations, Ultraviolet: Stars},
     year = 2001,
    month = nov,
   volume = 562,
    pages = {508-514},
      doi = {10.1086/323870},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...562..508M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1981ApJ...243..223H,
   author = {{Hildebrand}, R.~H. and {Spillar}, E.~J. and {Stiening}, R.~F.
	},
    title = "{Observations of fast oscillations in SS Cygni}",
  journal = {\apj},
 keywords = {COHERENT RADIATION, NOVAE, STELLAR OSCILLATIONS, STELLAR SPECTRA, STELLAR SPECTROPHOTOMETRY, ULTRAVIOLET RADIATION, WHITE DWARF STARS, LIGHT CURVE,
PHOTOMULTIPLIER TUBES, POWER SPECTRA, STELLAR LUMINOSITY, STELLAR MAGNITUDE, X RAY SOURCES},
     year = 1981,
    month = jan,
   volume = 243,
    pages = {223-227},
      doi = {10.1086/158587},
   adsurl = {http://adsabs.harvard.edu/abs/1981ApJ...243..223H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003MNRAS.344.1193W,
   author = {{Warner}, B. and {Woudt}, P.~A. and {Pretorius}, M.~L.},
    title = "{Dwarf nova oscillations and quasi-periodic oscillations in cataclysmic variables - III. A new kind of dwarf nova oscillation, and further examples of the
similarities to X-ray binaries}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/0306085},
 keywords = {accretion, accretion discs, stars: dwarf novae, novae, cataclysmic variables, stars: oscillations},
     year = 2003,
    month = oct,
   volume = 344,
    pages = {1193-1209},
      doi = {10.1046/j.1365-8711.2003.06905.x},
   adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.344.1193W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1974ApJ...189..315H,
   author = {{Hesser}, J.~E. and {Lasker}, B.~M. and {Osmer}, P.~S.},
    title = "{High-frequency stellar oscillations. X. The rapid blue variable CD -42 14452.}",
  journal = {\apj},
     year = 1974,
    month = apr,
   volume = 189,
    pages = {315-318},
      doi = {10.1086/152805},
   adsurl = {http://adsabs.harvard.edu/abs/1974ApJ...189..315H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002MNRAS.335...84W,
   author = {{Warner}, B. and {Woudt}, P.~A.},
    title = "{Dwarf nova oscillations and quasi-periodic oscillations in cataclysmic variables - II. A low-inertia magnetic accretor model}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/0204484},
 keywords = {accretion, accretion discs, stars: individual: VW Hyi, stars: individual: WZ Sge, stars: individual: V2051 Oph, novae, cataclysmic variables, stars:
oscillations},
     year = 2002,
    month = sep,
   volume = 335,
    pages = {84-98},
      doi = {10.1046/j.1365-8711.2002.05596.x},
   adsurl = {http://adsabs.harvard.edu/abs/2002MNRAS.335...84W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002PASP..114.1364P,
   author = {{Patterson}, J. and {Fenton}, W.~H. and {Thorstensen}, J.~R. and 
	{Harvey}, D.~A. and {Skillman}, D.~R. and {Fried}, R.~E. and 
	{Monard}, B. and {O'Donoghue}, D. and {Beshore}, E. and {Martin}, B. and 
	{Niarchos}, P. and {Vanmunster}, T. and {Foote}, J. and {Bolt}, G. and 
	{Rea}, R. and {Cook}, L.~M. and {Butterworth}, N. and {Wood}, M.
	},
    title = "{Superhumps in Cataclysmic Binaries. XXIII. V442 Ophiuchi and RX J1643.7+3402}",
  journal = {\pasp},
   eprint = {arXiv:astro-ph/0211615},
 keywords = {accretion, accretion disks, Stars: Binaries: Close, Stars: Novae, Cataclysmic Variables, stars: individual (V442 Ophiuchi), stars: individual (RX
J1643.7+3402)},
     year = 2002,
    month = dec,
   volume = 114,
    pages = {1364-1381},
      doi = {10.1086/344587},
   adsurl = {http://adsabs.harvard.edu/abs/2002PASP..114.1364P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1999ASPC..157....1H,
   author = {{Hellier}, C.},
    title = "{Recent results on intermediate polars}",
booktitle = {Annapolis Workshop on Magnetic Cataclysmic Variables},
     year = 1999,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 157,
   eprint = {arXiv:astro-ph/9901146},
   editor = {{Hellier}, C. and {Mukai}, K.},
    pages = {1},
   adsurl = {http://adsabs.harvard.edu/abs/1999ASPC..157....1H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1995ASPC...85..343W,
   author = {{Warner}, B.},
    title = "{DQ Herculis Stars and Dwarf Nova Oscillations}",
booktitle = {Magnetic Cataclysmic Variables},
     year = 1995,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 85,
   editor = {{Buckley}, D.~A.~H. and {Warner}, B.},
    pages = {343},
   adsurl = {http://adsabs.harvard.edu/abs/1995ASPC...85..343W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003AJ....125..348L,
   author = {{Liebert}, J. and {Bergeron}, P. and {Holberg}, J.~B.},
    title = "{The True Incidence of Magnetism Among Field White Dwarfs}",
  journal = {\aj},
   eprint = {arXiv:astro-ph/0210319},
 keywords = {Stars: Magnetic Fields, Stars: Statistics, Stars: White Dwarfs},
     year = 2003,
    month = jan,
   volume = 125,
    pages = {348-353},
      doi = {10.1086/345573},
   adsurl = {http://adsabs.harvard.edu/abs/2003AJ....125..348L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1978necb.conf...89P,
   author = {{Paczy{\'n}ski}, B.},
    title = "{Phenomenological Model of U Geminorum}",
booktitle = {Nonstationary Evolution of Close Binaries},
     year = 1978,
   editor = {{Zytkow}, A.~N.},
    pages = {89},
   adsurl = {http://adsabs.harvard.edu/abs/1978necb.conf...89P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1975ApJ...200..298K,
   author = {{Katz}, J.~I.},
    title = "{The structure of DQ Herculis.}",
  journal = {\apj},
     year = 1975,
    month = sep,
   volume = 200,
    pages = {298-305},
      doi = {10.1086/153788},
   adsurl = {http://adsabs.harvard.edu/abs/1975ApJ...200..298K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003MNRAS.345.1009W,
   author = {{Wheatley}, P.~J. and {West}, R.~G.},
    title = "{The X-ray eclipse of OY Car resolved with XMM-Newton: X-ray emission from the polar regions of the white dwarf}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/0307436},
 keywords = {accretion, accretion discs, binaries: eclipsing, stars: individual: OY Car, novae, cataclysmic variables, X-rays: stars},
     year = 2003,
    month = nov,
   volume = 345,
    pages = {1009-1014},
      doi = {10.1046/j.1365-8711.2003.07030.x},
   adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.345.1009W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1985ApJ...296..529C,
   author = {{Carroll}, B.~W. and {McDermott}, P.~N. and {Savedoff}, M.~P. and 
	{van Horn}, H.~M. and {Cabot}, W.},
    title = "{Accretion disk oscillations - A local analysis in a disk of finite thickness}",
  journal = {\apj},
 keywords = {ACCRETION DISKS, DWARF NOVAE, STELLAR MODELS, STELLAR OSCILLATIONS, GRAVITY WAVES, PERTURBATION, STABILITY, TWO DIMENSIONAL MODELS},
     year = 1985,
    month = sep,
   volume = 296,
    pages = {529-539},
      doi = {10.1086/163472},
   adsurl = {http://adsabs.harvard.edu/abs/1985ApJ...296..529C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000ApJ...534..934C,
   author = {{Collins}, T.~J.~B. and {Helfer}, H.~L. and {Van Horn}, H.~M.
	},
    title = "{Oscillations of Accretion Disks and Boundary Layers in Cataclysmic Variables. I. Unperturbed, Steady-Flow Models}",
  journal = {\apj},
 keywords = {Accretion, Accretion Disks, Stars: Novae, Cataclysmic Variables, Stars: White Dwarfs},
     year = 2000,
    month = may,
   volume = 534,
    pages = {934-943},
      doi = {10.1086/308771},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...534..934C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{rybicki2008radiative,
  title={Radiative Processes in Astrophysics},
  author={Rybicki, G.B. and Lightman, A.P.},
  isbn={9783527618187},
  series={Physics textbook},
  url={http://books.google.de/books?id=eswe2StAspsC},
  year={2008},
  publisher={John Wiley \& Sons}
}

@book{tucker1975radiation,
  title={Radiation processes in astrophysics},
  author={Tucker, W.H.},
  isbn={9780262700108},
  lccn={75029236},
  series={MIT Press Classics},
  url={http://books.google.de/books?id=FR81AQAAIAAJ},
  year={1975},
  publisher={MIT Press}
}

@book{landau1980statistical,
  title={Statistical Physics},
  author={Landau, L.D. and Lifshitz, E.M. and Sykes, J.B. and Kearsley, J.},
  isbn={9780750633727},
  lccn={78040140},
  series={Course of Theoretical Physics},
  url={http://books.google.de/books?id=kGGJuQAACAAJ},
  year={1980},
  publisher={Elsevier Science}
}

@ARTICLE{1994ApJ...428L..13N,
   author = {{Narayan}, R. and {Yi}, I.},
    title = "{Advection-dominated accretion: A self-similar solution}",
  journal = {\apjl},
   eprint = {arXiv:astro-ph/9403052},
 keywords = {ACCRETION DISKS, ADVECTION, ASTRONOMICAL MODELS, BLACK HOLES (ASTRONOMY), COOLING FLOWS (ASTROPHYSICS), STELLAR MASS ACCRETION, VISCOUS FLOW, HYDRODYNAMICS,
ROTATING DISKS, TWO DIMENSIONAL FLOW},
     year = 1994,
    month = jun,
   volume = 428,
    pages = {L13-L16},
      doi = {10.1086/187381},
   adsurl = {http://adsabs.harvard.edu/abs/1994ApJ...428L..13N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003ApJ...599..548D,
   author = {{D'Angelo}, G. and {Henning}, T. and {Kley}, W.},
    title = "{Thermohydrodynamics of Circumstellar Disks with High-Mass Planets}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0309236},
 keywords = {Accretion, Accretion Disks, Hydrodynamics, Methods: Numerical, Stars: Planetary Systems: Formation, Radiative Transfer},
     year = 2003,
    month = dec,
   volume = 599,
    pages = {548-576},
      doi = {10.1086/379224},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...599..548D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1990ApJ...351..632H,
   author = {{Hubeny}, I.},
    title = "{Vertical structure of accretion disks - A simplified analytical model}",
  journal = {\apj},
 keywords = {ACCRETION DISKS, ASTRONOMICAL MODELS, GRAY GAS, STELLAR ATMOSPHERES, STELLAR MASS ACCRETION, HYDROSTATICS, IRRADIATION, OPTICAL THICKNESS, THERMODYNAMIC
EQUILIBRIUM, VERTICAL DISTRIBUTION, VISCOUS DAMPING},
     year = 1990,
    month = mar,
   volume = 351,
    pages = {632-641},
      doi = {10.1086/168501},
   adsurl = {http://adsabs.harvard.edu/abs/1990ApJ...351..632H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005A&A...437..727K,
   author = {{Kley}, W. and {Lee}, M.~H. and {Murray}, N. and {Peale}, S.~J.
	},
    title = "{Modeling the resonant planetary system GJ 876}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0503579},
 keywords = {accretion, accretion disks, planets and satellites: formation, hydrodynamics, methods: N-body simulations},
     year = 2005,
    month = jul,
   volume = 437,
    pages = {727-742},
      doi = {10.1051/0004-6361:20052656},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...437..727K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{1985prpl.conf..981L,
   author = {{Lin}, D.~N.~C. and {Papaloizou}, J.},
    title = "{On the dynamical origin of the solar system}",
 keywords = {COMPUTATIONAL ASTROPHYSICS, INTERPLANETARY MEDIUM, PROTOSTARS, SOLAR SYSTEM, ACCRETION DISKS, ANGULAR MOMENTUM, CONVECTION, DENSITY DISTRIBUTION, GAS GIANT
PLANETS, NEBULAE, PLANETARY EVOLUTION, PROTOPLANETS},
booktitle = {Protostars and Planets II},
     year = 1985,
   editor = {{Black}, D.~C. and {Matthews}, M.~S.},
    pages = {981-1072},
   adsurl = {http://adsabs.harvard.edu/abs/1985prpl.conf..981L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@MASTERSTHESIS{Kolb2012,
	author = {{Kolb}, Stefan M.},
	title  = "{Dreidimensionaler Strahlungstransport in Zweitemperaturnäherung gekoppelt an den Code PLUTO}",
	school = {Eberhard Karls Universität Tübingen},
	year   = 2012,
	moth   = feb
}

@ARTICLE{Godunov59,
   author = {{Godunov}, S.~K.},
    title = "{A difference method for numerical calculation of discontinuous solutions of the equations of hydrodynamics}",
  journal = {Matematicheskii Sbornik (N.S.)},
     year = 1959,
    month = jun,
   volume = 47,
    pages = {271-306}
}

@ARTICLE{1977JCoPh..23..276V,
   author = {{van Leer}, B.},
    title = "{Towards the Ultimate Conservative Difference Scheme. IV. A New Approach to Numerical Convection}",
  journal = {J.~Comput.~Phys.},
     year = 1977,
    month = mar,
   volume = 23,
    pages = {276},
      doi = {10.1016/0021-9991(77)90095-X},
   adsurl = {http://adsabs.harvard.edu/abs/1977JCoPh..23..276V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1980ApJ...239..968N,
   author = {{Norman}, M.~L. and {Wilson}, J.~R. and {Barton}, R.~T.},
    title = "{A new calculation on rotating protostar collapse}",
  journal = {\apj},
 keywords = {ASTROPHYSICS, GRAVITATIONAL COLLAPSE, PLANETARY NEBULAE, PROTOSTARS, ADVECTION, ANGULAR MOMENTUM, ISOTHERMAL PROCESSES, ROTATING ENVIRONMENTS},
     year = 1980,
    month = aug,
   volume = 239,
    pages = {968-981},
      doi = {10.1086/158185},
   adsurl = {http://adsabs.harvard.edu/abs/1980ApJ...239..968N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Courant28,
   author = {{Courant}, R. and {Friedrichs}, K. and {Lewy}, H.},
    title = "{Über die partiellen Differnezengleichungen der mathematischen Physik}",
  journal = {Math.~Ann.},
     year = 1928,
    month = jun,
   volume = 100,
    pages = {32-74}
}

@book{richtmyer1967difference,
  title={Difference methods for initial-value problems},
  author={Richtmyer, R.D. and Morton, K.W.},
  lccn={lc67013959},
  series={Interscience tracts in pure and applied mathematics},
  url={http://books.google.de/books?id=WN5QAAAAMAAJ},
  year={1967},
  publisher={Interscience Publishers}
}

@ARTICLE{Thomas49,
   author = {{Thomas}, L.~H.},
    title = "{Elliptic problems in linear difference equations over a network}",
  journal = {Watson Sci. Comput. Lab. Rept. (Columbia University, New York)},
     year = 1949,
    month = jun
}

@ARTICLE{1950JAP....21..232V,
   author = {{Vonneumann}, J. and {Richtmyer}, R.~D.},
    title = "{A Method for the Numerical Calculation of Hydrodynamic Shocks}",
  journal = {J.~Appl.~Phys.},
     year = 1950,
    month = mar,
   volume = 21,
    pages = {232-237},
      doi = {10.1063/1.1699639},
   adsurl = {http://adsabs.harvard.edu/abs/1950JAP....21..232V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1979CoPhC..18..171T,
   author = {{Tscharnuter}, W.~M. and {Winkler}, K.-H.~A.},
    title = "{A method for computing selfgravitating gas flows with radiation.}",
  journal = {Comput.~Phys.~Commun.},
 keywords = {Mathematics, Computing, Data Processing},
     year = 1979,
   volume = 18,
    pages = {171-199},
      doi = {10.1016/0010-4655(79)90111-5},
   adsurl = {http://adsabs.harvard.edu/abs/1979CoPhC..18..171T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010A&A...511A..81K,
   author = {{Kuiper}, R. and {Klahr}, H. and {Dullemond}, C. and {Kley}, W. and 
	{Henning}, T.},
    title = "{Fast and accurate frequency-dependent radiation transport for hydrodynamics simulations in massive star formation}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1001.3301},
 primaryClass = "astro-ph.SR",
 keywords = {radiative transfer, hydrodynamics, stars: formation, circumstellar matter, accretion, accretion disks, methods: numerical},
     year = 2010,
    month = feb,
   volume = 511,
      eid = {A81},
    pages = {A81},
      doi = {10.1051/0004-6361/200912355},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...511A..81K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{1986rpa..book.....R,
   author = {{Rybicki}, G.~B. and {Lightman}, A.~P.},
    title = "{Radiative Processes in Astrophysics}",
booktitle = {Radiative Processes in Astrophysics, by George B.~Rybicki, Alan P.~Lightman, pp.~400.~ISBN 0-471-82759-2.~Wiley-VCH , June 1986.},
     year = 1986,
    month = jun,
   adsurl = {http://adsabs.harvard.edu/abs/1986rpa..book.....R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1992SvAL...18..104S,
   author = {{Suleymanov}, V.~F.},
    title = "{Modeling of the accretion disks and spectra of their radiation in cataclysmic variable stars. I - V603 AQL}",
  journal = {Soviet Astronomy Letters},
 keywords = {ACCRETION DISKS, CATACLYSMIC VARIABLES, STELLAR ATMOSPHERES, STELLAR MODELS, STELLAR SPECTRA, WHITE DWARF STARS, ATMOSPHERIC TEMPERATURE, STELLAR MAGNETIC
FIELDS, TEMPERATURE DISTRIBUTION},
     year = 1992,
    month = mar,
   volume = 18,
    pages = {104},
   adsurl = {http://adsabs.harvard.edu/abs/1992SvAL...18..104S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1985A&A...143...59R,
   author = {{Rozyczka}, M.},
    title = "{Two-dimensional models of stellar wind bubbles. I - Numerical methods and their application to the investigation of outer shell instabilities}",
  journal = {\aap},
 keywords = {COMPUTATIONAL FLUID DYNAMICS, INTERSTELLAR MATTER, MAGNETOHYDRODYNAMIC STABILITY, PLASMA BUBBLES, STELLAR ENVELOPES, STELLAR WINDS, TWO DIMENSIONAL MODELS,
HERBIG-HARO OBJECTS, MOLECULAR FLOW, NEBULAE, NONADIABATIC THEORY, PERTURBATION, RADIATIVE HEAT TRANSFER, STELLAR MODELS, THIN WALLED SHELLS},
     year = 1985,
    month = feb,
   volume = 143,
    pages = {59-71},
   adsurl = {http://adsabs.harvard.edu/abs/1985A%26A...143...59R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{kreiss1989initial,
  title={Initial-boundary value problems and the Navier-Stokes equations},
  author={Kreiss, H.O. and Lorenz, J.},
  isbn={9780080874562},
  series={Pure and Applied Mathematics},
  url={http://books.google.de/books?id=aCEq9TaC1tQC},
  year={1989},
  publisher={Elsevier Science}
}

@article{nordstrom2005well,
  title={Well-Posed Boundary Conditions for the Navier--Stokes Equations},
  author={Nordstr{\"o}m, Jan and Sv{\"a}rd, Magnus},
  journal={SIAM Journal on Numerical Analysis},
  volume={43},
  number={3},
  pages={1231--1255},
  year={2005},
  publisher={SIAM}
}

@PHDTHESIS{birken2012,
	author = {Birken, Philipp},
	pages = "217",
	title = "{N}umerical {M}ethods for the {U}nsteady {C}ompressible {N}avier-{S}tokes {E}quations",
	school = "University of Kassel",
	type = "{P}rofessorial dissertation",
	year = "2012",
	address = "Germany",
}

@ARTICLE{2007ApJ...662..564B,
   author = {{Bitner}, M.~A. and {Robinson}, E.~L. and {Behr}, B.~B.},
    title = "{The Masses and Evolutionary State of the Stars in the Dwarf Nova SS Cygni}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0703087},
 keywords = {Stars: Binaries: Close, Stars: Fundamental Parameters, Stars: Individual: Constellation Name: SS Cygni},
     year = 2007,
    month = jun,
   volume = 662,
    pages = {564-573},
      doi = {10.1086/517496},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...662..564B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1972ApJ...175..417N,
   author = {{Nauenberg}, M.},
    title = "{Analytic Approximations to the Mass-Radius Relation and Energy of Zero-Temperature Stars}",
  journal = {\apj},
     year = 1972,
    month = jul,
   volume = 175,
    pages = {417},
      doi = {10.1086/151568},
   adsurl = {http://adsabs.harvard.edu/abs/1972ApJ...175..417N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010ApJ...716L.157S,
   author = {{Sion}, E.~M. and {Godon}, P. and {Myzcka}, J. and {Blair}, W.~P.
	},
    title = "{The Accreting White Dwarf in SS Cygni Revealed}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1007.3158},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion disks, novae, cataclysmic variables, white dwarfs},
     year = 2010,
    month = jun,
   volume = 716,
    pages = {L157-L160},
      doi = {10.1088/2041-8205/716/2/L157},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...716L.157S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007ApJ...665.1254B,
   author = {{Boley}, A.~C. and {Durisen}, R.~H. and {Nordlund}, {\AA}. and 
	{Lord}, J.},
    title = "{Three-Dimensional Radiative Hydrodynamics for Disk Stability Simulations: A Proposed Testing Standard and New Results}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0704.2532},
 keywords = {Accretion, Accretion Disks, Convection, Hydrodynamics, Instabilities, Solar System: Formation},
     year = 2007,
    month = aug,
   volume = 665,
    pages = {1254-1267},
      doi = {10.1086/519767},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...665.1254B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1981MNRAS.196....1C,
   author = {{Cordova}, F.~A. and {Jensen}, K.~A. and {Nugent}, J.~J.},
    title = "{The HEAO-1 soft X-ray survey of cataclysmic variable stars}",
  journal = {\mnras},
 keywords = {DWARF NOVAE, HEAO 1, NOVAE, VARIABLE STARS, X RAY ASTRONOMY, DWARF STARS, STELLAR LUMINOSITY, X RAY SOURCES},
     year = 1981,
    month = jul,
   volume = 196,
    pages = {1-12},
   adsurl = {http://adsabs.harvard.edu/abs/1981MNRAS.196....1C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1981ApJ...245..609C,
   author = {{Cordova}, F.~A. and {Mason}, K.~O. and {Nelson}, J.~E.},
    title = "{X-ray observations of selected cataclysmic variable stars using the Einstein Observatory}",
  journal = {\apj},
 keywords = {BINARY STARS, DWARF STARS, NOVAE, STELLAR RADIATION, VARIABLE STARS, X RAY SOURCES, EMISSION SPECTRA, HEAO 2, SPACEBORNE ASTRONOMY, STELLAR MAGNETIC FIELDS,
STELLAR MASS ACCRETION, STELLAR SPECTRA},
     year = 1981,
    month = apr,
   volume = 245,
    pages = {609-617},
      doi = {10.1086/158836},
   adsurl = {http://adsabs.harvard.edu/abs/1981ApJ...245..609C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1984MNRAS.206..879C,
   author = {{Cordova}, F.~A. and {Mason}, K.~O.},
    title = "{X-ray observations of a large sample of cataclysmic variable stars using the Einstein Observatory}",
  journal = {\mnras},
 keywords = {BINARY STARS, STELLAR SPECTRA, STELLAR SPECTROPHOTOMETRY, VARIABLE STARS, X RAY SPECTRA, DWARF NOVAE, RADIANT FLUX DENSITY, SPECTRAL ENERGY DISTRIBUTION,
STELLAR LUMINOSITY},
     year = 1984,
    month = feb,
   volume = 206,
    pages = {879-897},
   adsurl = {http://adsabs.harvard.edu/abs/1984MNRAS.206..879C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1977AcA....27..235T,
   author = {{Tylenda}, R.},
    title = "{The continuous radiation emitted by accretion discs in cataclysmic binaries - The dwarf nova SS CYG during outburst and the old novae V 603 AQL and RR
PIC}",
  journal = {\actaa},
 keywords = {BINARY STARS, NOVAE, STELLAR MASS ACCRETION, STELLAR MODELS, WHITE DWARF STARS, ASTRONOMICAL SPECTROSCOPY, CYGNUS CONSTELLATION, SPECTRAL ENERGY
DISTRIBUTION, X RAY SOURCES},
     year = 1977,
   volume = 27,
    pages = {235-249},
   adsurl = {http://adsabs.harvard.edu/abs/1977AcA....27..235T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1986SvAL...12..117S,
   author = {{Syunyaev}, R.~A. and {Shakura}, N.~I.},
    title = "{Disk Accretion onto a Weak Field Neutron Star - Boundary Layer Disk Luminosity Ratio}",
  journal = {Soviet Astronomy Letters},
     year = 1986,
    month = apr,
   volume = 12,
    pages = {117},
   adsurl = {http://adsabs.harvard.edu/abs/1986SvAL...12..117S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...760...22B,
   author = {{Belyaev}, M.~A. and {Rafikov}, R.~R. and {Stone}, J.~M.},
    title = "{Angular Momentum Transport and Variability in Boundary Layers of Accretion Disks Driven by Global Acoustic Modes}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1205.4009},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion disks, hydrodynamics, instabilities, waves},
     year = 2012,
    month = nov,
   volume = 760,
      eid = {22},
    pages = {22},
      doi = {10.1088/0004-637X/760/1/22},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...760...22B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000AJ....120.2649H,
   author = {{Harrison}, T.~E. and {McNamara}, B.~J. and {Szkody}, P. and 
	{Gilliland}, R.~L.},
    title = "{The Spectroscopic and Astrometric Parallaxes of Three Dwarf Novae: The Nature of the Secondary Stars of U Geminorum, SS Aurigae, and SS Cygni}",
  journal = {\aj},
 keywords = {Stars: Novae, Cataclysmic Variables, Stars: Fundamental Parameters, stars: individual (SS Aurigae), Stars: Individual: Constellation Name: SS Cygni, Stars:
Individual: Constellation Name: U Geminorum},
     year = 2000,
    month = nov,
   volume = 120,
    pages = {2649-2660},
      doi = {10.1086/316802},
   adsurl = {http://adsabs.harvard.edu/abs/2000AJ....120.2649H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1984PASP...96..988S,
   author = {{Szkody}, P. and {Mattei}, J.~A.},
    title = "{Analysis of the AAVSO light curves of 21 dwarf novae}",
  journal = {\pasp},
 keywords = {DWARF NOVAE, LIGHT CURVE, SPECTRUM ANALYSIS, VARIABLE STARS, ORBITAL ELEMENTS, STELLAR MASS},
     year = 1984,
    month = dec,
   volume = 96,
    pages = {988-995},
      doi = {10.1086/131464},
   adsurl = {http://adsabs.harvard.edu/abs/1984PASP...96..988S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1974ApJ...187L...5R,
   author = {{Rappaport}, S. and {Cash}, W. and {Doxsey}, R. and {McClintock}, J. and 
	{Moore}, G.},
    title = "{Possible Detection of Very Soft X-Rays from SS Cygni}",
  journal = {\apjl},
     year = 1974,
    month = jan,
   volume = 187,
    pages = {L5},
      doi = {10.1086/181378},
   adsurl = {http://adsabs.harvard.edu/abs/1974ApJ...187L...5R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1980ApJ...235..163C,
   author = {{Cordova}, F.~A. and {Chester}, T.~J. and {Tuohy}, I.~R. and 
	{Garmire}, G.~P.},
    title = "{Soft X-ray pulsations from SS Cygni}",
  journal = {\apj},
 keywords = {BINARY STARS, DWARF STARS, NOVAE, PULSED RADIATION, STELLAR SPECTROPHOTOMETRY, X RAY SOURCES, BLACK BODY RADIATION, BOUNDARY LAYER STABILITY, HEAO, LIGHT
CURVE, PULSE DURATION, STELLAR LUMINOSITY, STELLAR MODELS, X RAY SPECTRA},
     year = 1980,
    month = jan,
   volume = 235,
    pages = {163-176},
      doi = {10.1086/157621},
   adsurl = {http://adsabs.harvard.edu/abs/1980ApJ...235..163C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003MNRAS.345...49W,
   author = {{Wheatley}, P.~J. and {Mauche}, C.~W. and {Mattei}, J.~A.},
    title = "{The X-ray and extreme-ultraviolet flux evolution of SS Cygni throughout outburst}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/0306471},
 keywords = {accretion, accretion discs, binaries: close, stars: dwarf novae, stars: individual: SS Cygni, novae, cataclysmic variables},
     year = 2003,
    month = oct,
   volume = 345,
    pages = {49-61},
      doi = {10.1046/j.1365-8711.2003.06936.x},
   adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.345...49W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004ApJ...601.1100M,
   author = {{McGowan}, K.~E. and {Priedhorsky}, W.~C. and {Trudolyubov}, S.~P.
	},
    title = "{On the Correlated X-Ray and Optical Evolution of SS Cygni}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0310425},
 keywords = {Stars: Novae, Cataclysmic Variables, Stars: Individual: Constellation Name: SS Cygni, X-Rays: Stars},
     year = 2004,
    month = feb,
   volume = 601,
    pages = {1100-1108},
      doi = {10.1086/380758},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...601.1100M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009PASJ...61S..77I,
   author = {{Ishida}, M. and {Okada}, S. and {Hayashi}, T. and {Nakamura}, R. and 
	{Terada}, Y. and {Mukai}, K. and {Hamaguchi}, K.},
    title = "{Suzaku Observations of SS Cygni in Quiescence and Outburst}",
  journal = {\pasj},
 keywords = {accretion, accretion disks, plasmas, stars: dwarf novae, X-rays: individual (SS Cygni)},
     year = 2009,
    month = jan,
   volume = 61,
    pages = {77},
   adsurl = {http://adsabs.harvard.edu/abs/2009PASJ...61S..77I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004ApJ...610..422M,
   author = {{Mauche}, C.~W.},
    title = "{Chandra Low Energy Transmission Grating Spectrum of SS Cygni in Outburst}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0403691},
 keywords = {Accretion, Accretion Disks, Stars: Binaries: Close, Stars: Novae, Cataclysmic Variables, Stars: Individual: Constellation Name: SS Cygni, X-Rays: Binaries},
     year = 2004,
    month = jul,
   volume = 610,
    pages = {422-426},
      doi = {10.1086/421438},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...610..422M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012AstL...38..238R,
   author = {{Revnivtsev}, M.~G. and {Burenin}, R.~A. and {Tkachenko}, A.~Y. and 
	{Khamitov}, I.~M. and {Ak}, T. and {Merloni}, A. and {Pavlinsky}, M.~N. and 
	{Sunyaev}, R.~A.},
    title = "{On the change of the inner boundary of an optically thick accretion disk around white dwarfs using the dwarf nova SS Cyg as an example}",
  journal = {Astronomy Letters},
archivePrefix = "arXiv",
   eprint = {1204.0902},
 primaryClass = "astro-ph.GA",
 keywords = {accretion disks, fast variability, optical observations},
     year = 2012,
    month = apr,
   volume = 38,
    pages = {238-248},
      doi = {10.1134/S1063773712040044},
   adsurl = {http://adsabs.harvard.edu/abs/2012AstL...38..238R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1997A&A...328..247L,
   author = {{Liu}, B.~F. and {Meyer}, F. and {Meyer-Hofmeister}, E.},
    title = "{Evaporation of the accretion disk in dwarf novae during = quiescence}",
  journal = {\aap},
 keywords = {ACCRETION, ACCRETION DISK, CATACLYSMIC VARIABLES, STARS: WHITE DWARFS, STARS: CORONAE},
     year = 1997,
    month = dec,
   volume = 328,
    pages = {247-252},
   adsurl = {http://adsabs.harvard.edu/abs/1997A%26A...328..247L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012PASJ...64...88S,
   author = {{Saitou}, K. and {Tsujimoto}, M. and {Ebisawa}, K. and {Ishida}, M.
	},
    title = "{Suzaku X-Ray Observation of the Dwarf Nova Z Camelopardalis at the Onset of an Optical Outburst}",
  journal = {\pasj},
archivePrefix = "arXiv",
   eprint = {1202.6226},
 primaryClass = "astro-ph.HE",
 keywords = {stars: binaries: close, stars: dwarf novae, stars: individual (Z Camelopardalis), stars: novae, cataclysmic variables, X-rays: stars},
     year = 2012,
    month = aug,
   volume = 64,
    pages = {88},
   adsurl = {http://adsabs.harvard.edu/abs/2012PASJ...64...88S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1982ApJ...260..716C,
   author = {{Cordova}, F.~A. and {Mason}, K.~O.},
    title = "{High-velocity winds from a dwarf nova during outburst}",
  journal = {\apj},
 keywords = {DWARF NOVAE, STELLAR MASS EJECTION, STELLAR WINDS, ULTRAVIOLET SPECTRA, VARIABLE STARS, ABSORPTION SPECTRA, BINARY STARS, BURSTS, IUE, STELLAR LUMINOSITY,
STELLAR SPECTRA, WIND VELOCITY},
     year = 1982,
    month = sep,
   volume = 260,
    pages = {716-721},
      doi = {10.1086/160291},
   adsurl = {http://adsabs.harvard.edu/abs/1982ApJ...260..716C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1982A&A...113...76K,
   author = {{Klare}, G. and {Wolf}, B. and {Stahl}, O. and {Krautter}, J. and 
	{Vogt}, N. and {Wargau}, W. and {Rahe}, J.},
    title = "{IUE observations of dwarf novae during active phases}",
  journal = {\aap},
 keywords = {DWARF NOVAE, IUE, STELLAR MASS EJECTION, STELLAR SPECTRA, WHITE DWARF STARS, EUROPEAN SPACE AGENCY, INTERSTELLAR EXTINCTION, SPECTRAL ENERGY DISTRIBUTION},
     year = 1982,
    month = sep,
   volume = 113,
    pages = {76-84},
   adsurl = {http://adsabs.harvard.edu/abs/1982A%26A...113...76K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1997MNRAS.288..649D,
   author = {{Done}, C. and {Osborne}, J.~P.},
    title = "{The X-ray spectrum of the dwarf nova SS CYG in quiescence and outburst}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/9703036},
 keywords = {ACCRETION, ACCRETION DISCS, BINARIES: CLOSE, STARS: INDIVIDUAL: SS CYG, NOVAE, CATACLYSMIC VARIABLES, X-RAYS: STARS.},
     year = 1997,
    month = jul,
   volume = 288,
    pages = {649-664},
   adsurl = {http://adsabs.harvard.edu/abs/1997MNRAS.288..649D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011ApJ...736...17P,
   author = {{Puebla}, R.~E. and {Diaz}, M.~P. and {Hillier}, D.~J. and {Hubeny}, I.
	},
    title = "{A Method for the Study of Accretion Disk Emission in Cataclysmic Variables. I. The Model}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1105.0851},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion disks, novae, cataclysmic variables, stars: mass-loss, ultraviolet: general},
     year = 2011,
    month = jul,
   volume = 736,
      eid = {17},
    pages = {17},
      doi = {10.1088/0004-637X/736/1/17},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...736...17P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJS..199....7F,
   author = {{Froning}, C.~S. and {Long}, K.~S. and {G{\"a}nsicke}, B. and 
	{Szkody}, P.},
    title = "{A Survey of Far Ultraviolet Spectroscopic Explorer Observations of Cataclysmic Variables}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1112.1972},
 primaryClass = "astro-ph.GA",
 keywords = {accretion, accretion disks, binaries: close, novae, cataclysmic variables, ultraviolet: stars},
     year = 2012,
    month = mar,
   volume = 199,
      eid = {7},
    pages = {7},
      doi = {10.1088/0067-0049/199/1/7},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJS..199....7F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...751...48P,
   author = {{Pessah}, M.~E. and {Chan}, C.-k.},
    title = "{On Hydromagnetic Stresses in Accretion Disk Boundary Layers}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1111.4219},
 primaryClass = "astro-ph.HE",
 keywords = {accretion, accretion disks, instabilities, magnetohydrodynamics: MHD, turbulence},
     year = 2012,
    month = may,
   volume = 751,
      eid = {48},
    pages = {48},
      doi = {10.1088/0004-637X/751/1/48},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...751...48P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012MmSAI..83..539S,
   author = {{Sion}, E.~M. and {Godon}, P.},
    title = "{White dwarfs in cataclysmic variable stars: accretion physics and evolution.}",
  journal = {\memsai},
     year = 2012,
   volume = 83,
    pages = {539},
   adsurl = {http://adsabs.harvard.edu/abs/2012MmSAI..83..539S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1998ApJ...505..339L,
   author = {{Livio}, M. and {Pringle}, J.~E.},
    title = "{The Rotation Rates of White Dwarfs and Pulsars}",
  journal = {\apj},
 keywords = {STARS: NOVAE, CATACLYSMIC VARIABLES, STARS: PULSARS: GENERAL, STARS: NEUTRON, STARS: WHITE DWARFS},
     year = 1998,
    month = sep,
   volume = 505,
    pages = {339-343},
      doi = {10.1086/306153},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...505..339L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011A&A...529A..35C,
   author = {{Commer{\c c}on}, B. and {Teyssier}, R. and {Audit}, E. and 
  {Hennebelle}, P. and {Chabrier}, G.},
    title = "{Radiation hydrodynamics with adaptive mesh refinement and application to prestellar core collapse. I. Methods}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1102.1216},
 primaryClass = "astro-ph.IM",
 keywords = {hydrodynamics, radiative transfer, methods: numerical, stars: formation, ISM: kinematics and dynamics, stars: low-mass},
     year = 2011,
    month = may,
   volume = 529,
      eid = {A35},
    pages = {A35},
      doi = {10.1051/0004-6361/201015880},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...529A..35C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007ApJ...667..626K,
   author = {{Krumholz}, M.~R. and {Klein}, R.~I. and {McKee}, C.~F. and 
  {Bolstad}, J.},
    title = "{Equations and Algorithms for Mixed-frame Flux-limited Diffusion Radiation Hydrodynamics}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0611003},
 keywords = {Hydrodynamics, Methods: Numerical, Radiative Transfer},
     year = 2007,
    month = sep,
   volume = 667,
    pages = {626-643},
      doi = {10.1086/520791},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...667..626K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1986ApJS...61..479H,
   author = {{Hachisu}, I.},
    title = "{A versatile method for obtaining structures of rapidly rotating stars}",
  journal = {\apjs},
 keywords = {COMPUTATIONAL ASTROPHYSICS, SELF CONSISTENT FIELDS, STELLAR ROTATION, STELLAR STRUCTURE, ANGULAR MOMENTUM, EQUATIONS OF STATE, ITERATION, POLYTROPIC PROCESSES, WHITE DWARF STARS},
     year = 1986,
    month = jul,
   volume = 61,
    pages = {479-507},
      doi = {10.1086/191121},
   adsurl = {http://adsabs.harvard.edu/abs/1986ApJS...61..479H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1995MNRAS.275.1093G,
   author = {{Godon}, P. and {Regev}, O. and {Shaviv}, G.},
    title = "{One-dimensional time-dependent numerical modelling of accretion disc boundary layers}",
  journal = {\mnras},
 keywords = {ACCRETION, ACCRETION DISCS, METHODS: NUMERICAL, BINARIES: CLOSE},
     year = 1995,
    month = aug,
   volume = 275,
    pages = {1093-1101},
   adsurl = {http://adsabs.harvard.edu/abs/1995MNRAS.275.1093G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1992ApJ...399L.163B,
   author = {{Bertout}, C. and {Regev}, O.},
    title = "{Cool mass-losing boundary layers of T Tauri accretion disks}",
  journal = {\apjl},
 keywords = {ACCRETION DISKS, BOUNDARY LAYER PLASMAS, STELLAR MASS ACCRETION, T TAURI STARS, COMPUTATIONAL ASTROPHYSICS, RADIATIVE TRANSFER, STELLAR MASS EJECTION, STELLAR MODELS},
     year = 1992,
    month = nov,
   volume = 399,
    pages = {L163-L166},
      doi = {10.1086/186632},
   adsurl = {http://adsabs.harvard.edu/abs/1992ApJ...399L.163B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1995MNRAS.272...71R,
   author = {{Regev}, O. and {Bertout}, C.},
    title = "{Asymptotic models of accretion disc boundary layers}",
  journal = {\mnras},
 keywords = {ACCRETION, ACCRETION DISCS-BINARIES, CLOSE-WHITE DWARFS},
     year = 1995,
    month = jan,
   volume = 272,
    pages = {71-79},
   adsurl = {http://adsabs.harvard.edu/abs/1995MNRAS.272...71R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008NewAR..51..814B,
   author = {{Balbus}, S.~A. and {Lesaffre}, P.},
    title = "{The effects of Prandtl number on black hole accretion flows}",
  journal = {\nar},
     year = 2008,
    month = may,
   volume = 51,
    pages = {814-818},
      doi = {10.1016/j.newar.2008.03.010},
   adsurl = {http://adsabs.harvard.edu/abs/2008NewAR..51..814B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002A&A...387..605M,
   author = {{Masset}, F.~S.},
    title = "{The co-orbital corotation torque in a viscous disk: Numerical simulations}",
  journal = {\aap},
   eprint = {astro-ph/0205211},
 keywords = {stars: planetary systems: formation, stars: planetary systems: protoplanetary disks, stars: planetary systems, hydrodynamics, methods: numerical},
     year = 2002,
    month = may,
   volume = 387,
    pages = {605-623},
      doi = {10.1051/0004-6361:20020240},
   adsurl = {http://adsabs.harvard.edu/abs/2002A%26A...387..605M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013A&A...560A..56H,
   author = {{Hertfelder}, M. and {Kley}, W. and {Suleimanov}, V. and {Werner}, K.
  },
    title = "{The boundary layer in compact binaries}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1310.5012},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion disks, binaries: close, white dwarfs, methods: numerical, hydrodynamics},
     year = 2013,
    month = dec,
   volume = 560,
      eid = {A56},
    pages = {A56},
      doi = {10.1051/0004-6361/201322542},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...560A..56H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1994ApJ...427..987B,
   author = {{Bell}, K.~R. and {Lin}, D.~N.~C.},
    title = "{Using FU Orionis outbursts to constrain self-regulated protostellar disk models}",
  journal = {\apj},
   eprint = {astro-ph/9312015},
 keywords = {Accretion Disks, Ionization, Protostars, Star Formation, Stellar Mass Accretion, Stellar Models, Thermal Stability, Hydrogen Clouds, Radial Flow, Stellar Mass Ejection},
     year = 1994,
    month = jun,
   volume = 427,
    pages = {987-1004},
      doi = {10.1086/174206},
   adsurl = {http://adsabs.harvard.edu/abs/1994ApJ...427..987B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012A&A...539A..18M,
   author = {{M{\"u}ller}, T.~W.~A. and {Kley}, W.},
    title = "{Circumstellar disks in binary star systems. Models for {$\gamma$} Cephei and {$\alpha$} Centauri}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1112.1845},
 primaryClass = "astro-ph.EP",
 keywords = {accretion, accretion disks, protoplanetary disks, hydrodynamics, radiative transfer, methods: numerical, planets and satellites: formation},
     year = 2012,
    month = mar,
   volume = 539,
      eid = {A18},
    pages = {A18},
      doi = {10.1051/0004-6361/201118202},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...539A..18M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013ApJ...770...67B,
   author = {{Belyaev}, M.~A. and {Rafikov}, R.~R. and {Stone}, J.~M.},
    title = "{Angular Momentum Transport by Acoustic Modes Generated in the Boundary Layer. I. Hydrodynamical Theory and Simulations}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1212.0580},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion disks, hydrodynamics, instabilities, waves },
     year = 2013,
    month = jun,
   volume = 770,
      eid = {67},
    pages = {67},
      doi = {10.1088/0004-637X/770/1/67},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...770...67B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{gatski2013compressibility,
  title={Compressibility, Turbulence and High Speed Flow},
  author={Gatski, T.B. and Bonnet, J.P.},
  isbn={9780123973184},
  url={http://books.google.de/books?id=xRmzb-uH2yEC},
  year={2013},
  publisher={Elsevier Science}
}

@book{peyret1996handbook,
  title={Handbook of Computational Fluid Mechanics},
  author={Peyret, R.},
  isbn={9780125530101},
  lccn={99067072},
  url={http://books.google.de/books?id=-Y-hISaJiPUC},
  year={1996},
  publisher={Academic Press}
}

@article{fjortoft1950application,
  title={Application of Integral Theorems in Deriving Criteria of Stability for Laminar Flows and for the Baroclinic Circular Vortex},
  author={Fj{\o}rtoft, R.},
  journal={Geofys. Publ., Oslo},
  volume=17,
  year={1950}
}

@BOOK{2004hyst.book.....D,
   author = {{Drazin}, P.~G. and {Reid}, W.~H.},
    title = "{Hydrodynamic Stability}",
booktitle = {Hydrodynamic Stability, by P.~G.~Drazin and W.~H.~Reid, pp.~626.~ISBN 0521525411.~Cambridge, UK: Cambridge University Press, September 2004.},
     year = 2004,
    month = sep,
   adsurl = {http://adsabs.harvard.edu/abs/2004hyst.book.....D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010MNRAS.401..791S,
   author = {{Springel}, V.},
    title = "{E pur si muove: Galilean-invariant cosmological hydrodynamical simulations on a moving mesh}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0901.4107},
 primaryClass = "astro-ph.CO",
 keywords = {methods: numerical, galaxies: interactions, cosmology: dark matter},
     year = 2010,
    month = jan,
   volume = 401,
    pages = {791-851},
      doi = {10.1111/j.1365-2966.2009.15715.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.401..791S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1988MNRAS.231..795G,
   author = {{Glatzel}, W.},
    title = "{Sonic instabilities in supersonic shear flows}",
  journal = {\mnras},
 keywords = {Acoustic Instability, Kelvin-Helmholtz Instability, Shear Flow, Shear Layers, Sound Waves, Supersonic Flow, Computational Fluid Dynamics, Radio Jets (Astronomy), Solar Wind, Supersonic Speed, Vortex Sheets},
     year = 1988,
    month = apr,
   volume = 231,
    pages = {795-821},
   adsurl = {http://adsabs.harvard.edu/abs/1988MNRAS.231..795G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...752..115B,
   author = {{Belyaev}, M.~A. and {Rafikov}, R.~R.},
    title = "{Supersonic Shear Instabilities in Astrophysical Boundary Layers}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1112.3102},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion disks, hydrodynamics, instabilities, waves},
     year = 2012,
    month = jun,
   volume = 752,
      eid = {115},
    pages = {115},
      doi = {10.1088/0004-637X/752/2/115},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...752..115B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1984MNRAS.208..721P,
   author = {{Papaloizou}, J.~C.~B. and {Pringle}, J.~E.},
    title = "{The dynamical stability of differentially rotating discs with constant specific angular momentum}",
  journal = {\mnras},
 keywords = {Accretion Disks, Angular Momentum, Astronomical Models, Dynamic Stability, Rotating Fluids, Toruses, Eigenvalues, Perturbation Theory, Polytropic Processes, Quasars},
     year = 1984,
    month = jun,
   volume = 208,
    pages = {721-750},
   adsurl = {http://adsabs.harvard.edu/abs/1984MNRAS.208..721P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1987MNRAS.228....1N,
   author = {{Narayan}, R. and {Goldreich}, P. and {Goodman}, J.},
    title = "{Physics of modes in a differentially rotating system - Analysis of the shearing sheet}",
  journal = {\mnras},
 keywords = {Compressible Flow, Computational Astrophysics, Computational Fluid Dynamics, Rotating Fluids, Shear Layers, Two Dimensional Flow, Coriolis Effect, Density Distribution, Disk Galaxies, Protostars, Stellar Rotation},
     year = 1987,
    month = sep,
   volume = 228,
    pages = {1-41},
   adsurl = {http://adsabs.harvard.edu/abs/1987MNRAS.228....1N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1976ApJ...205..363M,
   author = {{Mark}, J.~W.~K.},
    title = "{On Density Waves in Galaxies. III. Wave Amplification by Stimulated Emission}",
  journal = {\apj},
     year = 1976,
    month = apr,
   volume = 205,
    pages = {363-378},
      doi = {10.1086/154287},
   adsurl = {http://adsabs.harvard.edu/abs/1976ApJ...205..363M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{2008gady.book.....B,
   author = {{Binney}, J. and {Tremaine}, S.},
    title = "{Galactic Dynamics: Second Edition}",
booktitle = {Galactic Dynamics: Second Edition, by James Binney and Scott Tremaine.~ISBN 978-0-691-13026-2 (HB).~Published by Princeton University Press, Princeton, NJ USA, 2008.},
     year = 2008,
publisher = {Princeton University Press},
   adsurl = {http://adsabs.harvard.edu/abs/2008gady.book.....B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@PHDTHESIS{2008PhDT.......292B,
   author = {{Baruteau}, C.},
    title = "{Toward predictive scenarios of planetary migration}",
 keywords = {planetary migration, protoplanetary discs, hydrodynamics},
   school = {CEA Saclay, Service d'Astrophysique, 91191 Gif/Yvette Cedex, France},
     year = 2008,
    month = {October},
   adsurl = {http://adsabs.harvard.edu/abs/2008PhDT.......292B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013A&A...560A..40M,
   author = {{M{\"u}ller}, T.~W.~A. and {Kley}, W.},
    title = "{Modelling accretion in transitional disks}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1310.4398},
 primaryClass = "astro-ph.EP",
 keywords = {accretion, accretion disks, protoplanetary disks, planet-disk interactions, methods: numerical, hydrodynamics, planets and satellites: formation},
     year = 2013,
    month = dec,
   volume = 560,
      eid = {A40},
    pages = {A40},
      doi = {10.1051/0004-6361/201322503},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...560A..40M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Article{Hunter:2007,
  Author    = {Hunter, J. D.},
  Title     = {Matplotlib: A 2D graphics environment},
  Journal   = {Computing In Science \& Engineering},
  Volume    = {9},
  Number    = {3},
  Pages     = {90--95},
  abstract  = {Matplotlib is a 2D graphics package used for Python
  for application development, interactive scripting, and
  publication-quality image generation across user
  interfaces and operating systems.},
  publisher = {IEEE COMPUTER SOC},
  year      = 2007
}

@INPROCEEDINGS{2014ASPC..488..127R,
   author = {{Romanova}, M. and {Kurosawa}, R.},
    title = "{Simulations of Accretion onto Magnetized Stars: Results of 3D MHD Simulations and 3D Radiative Transfer}",
booktitle = {8th International Conference of Numerical Modeling of Space Plasma Flows (ASTRONUM 2013)},
     year = 2014,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 488,
archivePrefix = "arXiv",
   eprint = {1401.4761},
 primaryClass = "astro-ph.SR",
   editor = {{Pogorelov}, N.~V. and {Audit}, E. and {Zank}, G.~P.},
    month = sep,
    pages = {127},
   adsurl = {http://adsabs.harvard.edu/abs/2014ASPC..488..127R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Velikhov_1959, 
  title={STABILITY OF AN IDEALLY CONDUCTING LIQUID FLOWING BETWEEN ROTATING CYLINDERS IN A MAGNETIC FIELD}, 
  abstractNote={Sufficient conditions for the stability of an ideal liquid flowing in axial and toroidal fields are derived.  Critical values of the magnetic fields which stabilize the flow are obtained and a physical interpretation of the results is presented.  (auth)}, 
  author={Velikhov, E.P.}, 
  year={1959}, 
  month={May},
  journal={Zhur. Eksptl. i Teoret. Fiz.},
  volume={36}
}

@ARTICLE{1960PNAS...46..253C,
   author = {{Chandrasekhar}, S.},
    title = "{The Stability of Non-Dissipative Couette Flow in Hydromagnetics}",
  journal = {Proceedings of the National Academy of Science},
     year = 1960,
    month = feb,
   volume = 46,
    pages = {253-257},
      doi = {10.1073/pnas.46.2.253},
   adsurl = {http://adsabs.harvard.edu/abs/1960PNAS...46..253C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1993ApJ...419..768F,
   author = {{Fujimoto}, M.~Y.},
    title = "{The Evolution of Accreting Stars with Turbulent Mixing}",
  journal = {\apj},
 keywords = {ACCRETION, ACCRETION DISKS, STARS: EVOLUTION, STARS: INTERIORS, STARS: NOVAE, CATACLYSMIC VARIABLES, TURBULENCE, X-RAYS: BURSTS},
     year = 1993,
    month = dec,
   volume = 419,
    pages = {768},
      doi = {10.1086/173528},
   adsurl = {http://adsabs.harvard.edu/abs/1993ApJ...419..768F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1973MNRAS.161..365T,
   author = {{Tayler}, R.~J.},
    title = "{The adiabatic stability of stars containing magnetic fields-I.Toroidal fields}",
  journal = {\mnras},
     year = 1973,
   volume = 161,
    pages = {365},
   adsurl = {http://adsabs.harvard.edu/abs/1973MNRAS.161..365T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2002A&A...381..923S,
   author = {{Spruit}, H.~C.},
    title = "{Dynamo action by differential rotation in a stably stratified stellar interior}",
  journal = {\aap},
   eprint = {astro-ph/0108207},
 keywords = {MAGNETOHYDRODYNAMICS (MHD), STARS: MAGNETIC FIELDS, INSTABILITIES},
     year = 2002,
    month = jan,
   volume = 381,
    pages = {923-932},
      doi = {10.1051/0004-6361:20011465},
   adsurl = {http://adsabs.harvard.edu/abs/2002A%26A...381..923S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013ApJ...770...68B,
   author = {{Belyaev}, M.~A. and {Rafikov}, R.~R. and {Stone}, J.~M.},
    title = "{Angular Momentum Transport by Acoustic Modes Generated in the Boundary Layer. II. Magnetohydrodynamic Simulations}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1301.4573},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion disks, instabilities, magnetohydrodynamics: MHD, waves },
     year = 2013,
    month = jun,
   volume = 770,
      eid = {68},
    pages = {68},
      doi = {10.1088/0004-637X/770/1/68},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...770...68B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1993ApJ...418L..71H,
   author = {{Hayashi}, M. and {Ohashi}, N. and {Miyama}, S.~M.},
    title = "{A Dynamically Accreting Gas Disk around HL Tauri}",
  journal = {\apjl},
 keywords = {ISM: JETS AND OUTFLOWS, STARS: FORMATION, STARS: PRE-MAIN-SEQUENCE},
     year = 1993,
    month = dec,
   volume = 418,
    pages = {L71},
      doi = {10.1086/187119},
   adsurl = {http://adsabs.harvard.edu/abs/1993ApJ...418L..71H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1999ApJ...521..650B,
   author = {{Balbus}, S.~A. and {Papaloizou}, J.~C.~B.},
    title = "{On the Dynamical Foundations of {$\alpha$} Disks}",
  journal = {\apj},
   eprint = {astro-ph/9903035},
 keywords = {ACCRETION, ACCRETION DISKS, HYDRODYNAMICS, INSTABILITIES, TURBULENCE, Accretion, Accretion Disks, Hydrodynamics, Instabilities, Turbulence},
     year = 1999,
    month = aug,
   volume = 521,
    pages = {650-658},
      doi = {10.1086/307594},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...521..650B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1978JQSRT..20..541M,
   author = {{Minerbo}, G.~N.},
    title = "{Maximum entropy Eddington factors.}",
  journal = {\jqsrt},
 keywords = {Radiative Transfer},
     year = 1978,
   volume = 20,
    pages = {541-545},
      doi = {10.1016/0022-4073(78)90024-9},
   adsurl = {http://adsabs.harvard.edu/abs/1978JQSRT..20..541M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013A&A...549A.124B,
   author = {{Bitsch}, B. and {Crida}, A. and {Morbidelli}, A. and {Kley}, W. and 
	{Dobbs-Dixon}, I.},
    title = "{Stellar irradiated discs and implications on migration of embedded planets. I. Equilibrium discs}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1211.6345},
 primaryClass = "astro-ph.EP",
 keywords = {accretion, accretion disks, planets and satellites: formation, hydrodynamics, radio continuum: galaxies, radiative transfer, planet-disk interactions},
     year = 2013,
    month = jan,
   volume = 549,
      eid = {A124},
    pages = {A124},
      doi = {10.1051/0004-6361/201220159},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...549A.124B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015A&A...579A..54H,
   author = {{Hertfelder}, M. and {Kley}, W.},
    title = "{Wave mediated angular momentum transport in astrophysical boundary layers}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1505.01714},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion disks, hydrodynamics, instabilities, waves, methods: numerical, stars: protostars},
     year = 2015,
    month = jul,
   volume = 579,
      eid = {A54},
    pages = {A54},
      doi = {10.1051/0004-6361/201526005},
   adsurl = {http://adsabs.harvard.edu/abs/2015A%26A...579A..54H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007ApJS..170..228M,
   author = {{Mignone}, A. and {Bodo}, G. and {Massaglia}, S. and {Matsakos}, T. and 
	{Tesileanu}, O. and {Zanni}, C. and {Ferrari}, A.},
    title = "{PLUTO: A Numerical Code for Computational Astrophysics}",
  journal = {\apjs},
   eprint = {astro-ph/0701854},
 keywords = {Hydrodynamics, Methods: Numerical, Magnetohydrodynamics: MHD, Relativity, Shock Waves},
     year = 2007,
    month = may,
   volume = 170,
    pages = {228-242},
      doi = {10.1086/513316},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJS..170..228M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013A&A...559A..80K,
   author = {{Kolb}, S.~M. and {Stute}, M. and {Kley}, W. and {Mignone}, A.
	},
    title = "{Radiation hydrodynamics integrated in the PLUTO code}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1309.5231},
 primaryClass = "astro-ph.EP",
 keywords = {radiative transfer, hydrodynamics, accretion, accretion disks},
     year = 2013,
    month = nov,
   volume = 559,
      eid = {A80},
    pages = {A80},
      doi = {10.1051/0004-6361/201321499},
   adsurl = {http://adsabs.harvard.edu/abs/2013A%26A...559A..80K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016ApJ...817...62P,
   author = {{Philippov}, A.~A. and {Rafikov}, R.~R. and {Stone}, J.~M.},
    title = "{Spreading Layers in Accreting Objects: Role of Acoustic Waves for Angular Momentum Transport, Mixing, and Thermodynamics}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1511.09115},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion disks, hydrodynamics, instabilities, waves},
     year = 2016,
    month = jan,
   volume = 817,
      eid = {62},
    pages = {62},
      doi = {10.3847/0004-637X/817/1/62},
   adsurl = {http://adsabs.harvard.edu/abs/2016ApJ...817...62P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2016arXiv161004289B,
   author = {{Belyaev}, M.},
    title = "{Incompressible Modes Excited by Supersonic Shear in Boundary Layers: Acoustic CFS Instability}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1610.04289},
 primaryClass = "astro-ph.HE",
 keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
     year = 2016,
    month = oct,
   adsurl = {http://adsabs.harvard.edu/abs/2016arXiv161004289B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014a&a...571a..55s,
   author = {{Suleimanov}, V. and {Hertfelder}, M. and {Werner}, K. and {Kley}, W.
	},
    title = "{Modeling the EUV spectra of optically thick boundary layers of dwarf novae in outburst}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1408.4369},
 primaryClass = "astro-ph.SR",
 keywords = {accretion, accretion disks, stars: dwarf novae, radiative transfer, methods: numerical, X-rays: binaries},
     year = 2014,
    month = nov,
   volume = 571,
      eid = {A55},
    pages = {A55},
      doi = {10.1051/0004-6361/201423724},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...571A..55S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

